Non-Symmetric Coded Caching for Location-Dependent Content Delivery

Immersive viewing is emerging as the next interface evolution for human-computer interaction. A truly wireless immersive application necessitates immense data delivery with ultra-low latency, raising stringent requirements for next-generation wireless networks. A potential solution for addressing these requirements is through the efficient usage of in-device storage and computation capabilities. This paper proposes a novel location-based coded cache placement and delivery scheme, which leverages the nested code modulation (NCM) to enable multi-rate multicasting transmission. To provide a uniform quality of experience in different network locations, we formulate a linear programming cache allocation problem. Next, based on the users' spatial realizations, we adopt an NCM based coded delivery algorithm to efficiently serve a distinct group of users during each transmission. Numerical results demonstrate that the proposed location-based delivery method significantly increases transmission efficiency compared to state of the art.

==> Figures/Data/Fig23.tex <==
States	rates	Memory
1	3	25
2	2	50
3	1	75
4	2	50
5	3	25


==> Figures/Data/Fig4.tex <==
K	Tu	Tx	Tm
2.00	22.417	13.0839	11.2092
4.00	44.834	14.5858	14.797
6.00	67.251	17.0666	14.394
8.00	89.668	17.6221	14.9472
10.00	112.085	19.5806	15.675
12.00	134.502	19.6288	15.8259
14.00	156.919	20.5986	15.8379
16.00	179.336	20.5849	16.1166
18.00	201.753	20.9576	16.2863
20.00	224.17	21.0379	16.5118
22.00	246.587	21.4939	16.3505
24.00	269.004	21.9699	16.5005
26.00	291.421	21.8099	16.6903
28.00	313.838	22.3583	16.6137
30.00	336.255	22.5763	16.5929
32.00	358.672	22.3293	16.8354
34.00	381.089	22.7776	16.9614
36.00	403.506	22.4904	16.6834
38.00	425.923	22.8297	16.8527
40.00	448.34	22.9195	17.032


==> Figures/Data/Fig56.tex <==
M	Tu-Tm-S121	Tu-Tx-S121	Tu-Tm-S441	Tu-Tx-S441
0.0	1.00	1.00	1.00	1.00
0.1	1.125	1.715	1.1005	0.9352
0.2	1.4204	2.3821	1.2627	0.9259
0.3	1.8646	3.0289	1.4379	0.9054
0.4	2.5103	3.6647	1.5884	0.8623
0.5	3.7638	4.2871	1.8446	0.8065
0.6	5.2718	4.8986	2.06360	0.7465
0.7	6.5411	5.501	2.5547	0.6907
0.8	7.998	6.0954	3.1313	0.6663
0.9	8.996	6.6831	6.7314	0.7047


==> Figures/Fig_mem.tex <==
%\begin{figure}
    \centering
    \resizebox{\columnwidth}{!}{%

    \begin{tikzpicture}

    \begin{axis}
    [
    % put axis lines at left and bottom
    axis lines = left,
    % control axis labels
    xlabel near ticks,
    xlabel = \smaller {States},
    ylabel = \smaller {\% memory},
    ylabel near ticks,
    ymin = 0, %ymax = 20,
    % control legend position
    %legend pos = north west,
    % control size of tick marks (10,20,30,etc)
    ticklabel style={font=\smaller},
    % control major grids
    grid=both,
    major grid style={line width=.2pt,draw=gray!30},
    % control minor grids
    %grid style={line width=.1pt, draw=gray!10},
    %minor tick num=5,
    %ybar interval=0.7,
    ]
    
    \addplot
    [mark = square, black]
    table[y=Memory,x=States]{Figures/Data/Fig23.tex};
    %\addlegendentry{\tiny $T_u$}
    
    \end{axis}

    \end{tikzpicture}
    }

    \caption{Location-specific memory distribution.
    }
    \label{fig:cache_distribution}
%\end{figure}

==> LiteratureRev.tex <==
Sample citation~\cite{maddah2014fundamental}.

\begin{itemize}
    \item Coded caching
    \item Wireless coded caching
    \item Coded caching with uneven cache placement (?)
    \item Caching applications in immersive viewing
\end{itemize}

==> NewScheme.tex <==
Similar to other coded caching schemes in the literature, our new NCM-based scheme also works in two distinct phases, cache placement and content delivery. For better clarification, throughout the discussions we frequently refer to the example network considered in Section~\ref{section:example_net}.
%However, the cache placement phase itself is performed in two steps: memory allocation and pool arrangement.

%The NCM-based cache placement is performed in two sub-phases: location-based cache portion allocation and cache pool arrangement. For the first phase, based on each specific location rate, we aim to minimize the maximum delivery time for all the states. In this manner, we aim to provide the minimum achievable delivery time for each state based on the fact that all the states have the same access probability. 

\subsection{Cache Placement}
For cache placement, we first determine the amount of cache memory (at every user) allocated to storing $F^i$, where $F^i$ is the file required for the user $u_i$ located at state $s_i$, $i \in \CS$. During this memory allocation process, we aim to minimize the maximum delivery time for all the states, assuming that all the states have the same access probability. From the system model, we know that the size of each $F^i$ is $F$ data units, and hence, if every user $u_j$ dedicates $m_iF$ data units in its cache memory for storing $F^i$, $F-m_iF$ data units should be delivered over the communication channel. As the result, if the single-user achievable rate at state $s_i$ is equal to $r_i$, the total delivery time for this state is $T_i = \frac{F-m_iF}{r_i}$. Finally, memory allocation for minimizing the maximum delivery time can be found by solving the following linear programming problem

%In general, at the state $s \in \mathcal{S}$ the total amount of $F_s$ [bits/Hz/s] needs to be delivered for the users located in this state. Since each user $k$ dedicates $m_s$ portion of its memory to cache some portion of the required data for this location, $F_s - m_s$ remaining data must be delivered to the user $k$ in state $s$ with available rate $r_s$. Therefore, the total required time to serve a user at state $s$ is $T_s = \frac{F_s - m_s}{r_s}$. Since all the states have the same access probability, there is no priority for any state. In this regard, we aim to allocate the memory portion to states such that the maximum delivery time among all the states is minimized. Note that each user has a limited memory of size $MF$ [bits/Hz]. Therefore, the memory allocation problem can be formulated to a LP as follows

\begin{equation}
\begin{aligned}
\label{cache-allocation}
 \text{LP} \ : \quad &\min_{\{m_i\}, \gamma}  \gamma\\
&\textrm{s.t.} \quad  \frac{F-m_iF}{r_i} \leq \gamma, \ \forall i \in \CS, \\
& \sum_{i \in \CS} m_i = M,\\
& m_i \geq 0, \ \forall i \in \CS, \\
& \gamma \geq 0.
\end{aligned}
\end{equation}

By solving~\eqref{cache-allocation}, the amount of cache memory (at every user) dedicated to each state is determined. Next, we arrange all the users' memory based on cache placement proposed in~\cite{maddah2014fundamental}. Note that in our proposed method, required files in each state are considered as a separate library, and the algorithm in~\cite{maddah2014fundamental} is performed for each state independent of the other states.
%\subsection{Cache Placement}
%Cache placement for each state follows the original coded caching scheme proposed in~\cite{maddah2014fundamental}. 
In this regard, $F^i$ is partitioned into $\binom{K}{t_i}$ parts denoted by $f^{i}_{\CV_i}$, where $\CV_i$ denotes a subset of users with $|\CV_i| = t_i$, and $t_i = Km_i$. Then, every user $k \in \CK$ fills up its cache as
\begin{equation}
    \CZ_k = \{f^{i}_{\CV_i} | \ \forall i, \forall \CV_i \ni k \} \; .
\end{equation}
%with some parts from all the states such that $\mathcal{Z}_k = \{f^{s}_{\CV} | \ \forall \CV, \  k \in \CV, \forall s\}$.

It can be easily verified that this cache placement satisfies the memory constraints. This is due to the fact that 
%\begin{theorem}
%The proposed cache placement satisfies the memory constraint.
%\begin{proof}
at each state $s_i$ the required file $F^i$ is divided into $\binom{K}{t_i}$ parts. Each user $k \in \CK$ stores $\binom{K-1}{t_i-1}$ of these parts, and hence, the total memory dedicated to state $s_i$ is
\begin{equation}
    \frac{\binom{K-1}{t_i-1}F^i}{\binom{K}{t_i}}=\frac{t_i F^i}{K} \; .
\end{equation}
data bits. Now, replacing $t_i$ with $K m_i$ and summing over all the states, we get $\sum_{s_i \in \CS}m_i F^i = MF$.
%\end{proof}
%\end{theorem}

\begin{algorithm}
	\caption{Location-based Cache Placement\label{Alg_Main}}
	\begin{algorithmic}[1]
		
%		\Procedure{MEM\_ALLOC}%{$\{ F^i, r_i ; \forall s_i \in \CS \}$}
		
%		\State $\mathcal{M} =  \arg\min\limits_{\CM = \{m_i\}}\max\limits_{i} \frac{F^i-m_i}{r_i} $
		%= \left\{m_{s_i} \bigg| \frac{F_s-m_{s}}{r_{s}}|_{s=s_i} = \min\limits_{\{m_{s^{'}}\}} \max \frac{F_{s_{'}}-m_{s^{'}}}{r_{s^{'}}}, \ \sum\limits_{s \in \mathcal{S}}m_s = M \right\}$
%		\EndProcedure
%	\end{algorithmic}
%\end{algorithm*}
%
%\begin{algorithm*}
%	\begin{algorithmic}[1]
		\Procedure{CACHE\_PLACEMENT}{}%{$\{ F^i, r_i ; \forall s_i \in \CS \}, \CK$}
		\State $\{m_i \} =  \arg\min\max\limits_{i} \frac{F-m_i F}{r_i} $
		
		\For{$s_i\in\mathcal{S}$} %\Comment{This is the beginning cache-arrangement.}
		
		\State $t_i = K \times m_i$ 
		
		\State $F^i \rightarrow \{f^{i}_{\CV_i} \; | \; \CV_i \subseteq \CK, |\CV_i| = t_i\}$
		
		\For{$k \in \CK$}
		\If{$k \in \CV$}
		    \State $\CZ_k \gets f^{i}_{\CV}$
		\EndIf
		\EndFor
		\EndFor
		\EndProcedure %\Comment{ This is the end of cache placement phase.}
	\end{algorithmic}
\end{algorithm}

\begin{algorithm}
    \caption{NCM-based Content Delivery}
	\begin{algorithmic}[1]
		\Procedure{DELIVERY}{}
		%{$\{F_{s_i},\dots,F_{s_j}\}$, \ $\{r_{s_i}, \ldots, r_{s_j}\}, \ \{\mathcal{Z}_1, \dots, \mathcal{Z}_K\}$}
		
		\State $t_c = \min\limits_{s_i \in \CS_u} t_i$
		\ForAll{$\CV_c \subseteq \CK, |\CV_c| = t_c+1$}
		    \State $X_c \gets 0$
		    \ForAll{$u_j \in \CV_c$}
		        \State $\alpha_j \gets \binom{t_j}{t_c}$
		        \State $Y_j \gets 0$
		        \State $\CV_{c \backslash j} = \CV_c \backslash \{u_j \}$
		        \ForAll{$\CV_j \subseteq \CK, |\CV_j| = t_j+1$}
		            \If{$\CV_{c \backslash j} \subseteq \CV_j$}
		                \State $f^{j,q}_{\CV_j} \gets$ \textsc{NewChunk}($f^{j}_{\CV_j}, \alpha_j$)
		                \State $Y_j \gets$ \textsc{Concatenate} $ (Y_j, f^{j,q}_{\CV_j})$ 
		            \EndIf
		        \EndFor
		        \State $X_c \gets$ \textsc{Nest} $(X_c, Y_j, r_j)$
		    \EndFor
		    \State Transmit $X_c$
		\EndFor
		
		%\State
		
		%\ForAll{$ s_i \in \CS_{u}$}
		%\ForAll{$ \CV \subseteq \CK, |\CV| = t_c$}
		%\State $\hat{f}^{s_i}_{\CV} = [NEW({f^{s_i}_{\CV_s}})]_{\{\forall \CV_s | \CV \subseteq \CV_s\}}$ 
		%\State \Comment{The function $NEW({f^{s}_{\mathcal{V}_s}})$ chooses a new part of $f^{s}_{\mathcal{V}_s}$ with size $\frac{|f^{s}_{\mathcal{V}_s}|}{\binom{t_s}{t_c}}$, and $[.]$ denotes concatenation.}
		%\EndFor
		%\EndFor
		
		%\ForAll{$\CD \subseteq \CK, |\CD|= t_c + 1$}

		%\State $X_{\CD} \gets *_{k \in \CD} f^{s_{u_k}}_{\CD \setminus k} $ 
		%\State \Comment{Nest each $f^{s_{u_k}}_{\CD \setminus k}$ together and transmit each file with the corresponding rate.}
		%\EndFor
		
		%\State \textbf{Transmit} $f^{s_{u_k}}_{\mathcal{D} \setminus k}$ with the rate $r_{s_{u_k}}$.
		\EndProcedure
		
	\end{algorithmic}
\end{algorithm}

\subsection{Content Delivery}
In the delivery phase, each user $u_j \in \CK$ is at a particular state $s_j \in \CS$. Based on the proposed cache placement, each state $s_j$ has specific $t_j$ and $r_j$ values. We set the common multicasting factor $t_c$ to be the minimum of $t_j$ values for all the users, i.e., $t_c = \min\limits_{u_j \in \CK}t_j$.

We deliver a nested codeword $X_{\CV_c}$ to any subset of users $\CV_c$ with size $t_c+1$ users. This nested codeword is designed such that the users with higher data rates (with smaller $t_j$ values) receive a larger data portion. Note that every user $u_j \in \CV_c$ has cached data parts $f^j_{\CV_j}$ for which $u_j \in \CV_j$, and needs to receive the rest of these data parts for a successful delivery. Let us denote the user set $\CV_c \backslash \{u_j\}$ with $\CV_{c \backslash j}$. During the transmission of $X_{\CV_c}$, we can deliver all data part(s) $f^j_{\CV_j}$ to $u_j$, for which $\CV_{c \backslash j} \subseteq \CV_j$. However, delivering all such data parts all together with $X_{\CV_c}$ causes $X_{\CV_c}$ to be \textit{inefficient}, i.e., there will be time instances during the transmission of $X_{\CV_c}$ in which some users in $\CV_c$ are not receiving any data. To solve this issue, we split every data part $f^j_{\CV_j}$ for which  $\CV_{c \backslash j} \subseteq \CV_j$ into smaller chunks, by splitting them into $\binom{t_j}{t_c}$ chunks denoted with $f^{j,q}_{\CV_j}$, where $q$ is an auxiliary index used to avoid transmitting the same data chunk multiple times. Finally, we concatenate all these data chunks.


In order to do so, for every user $u_j \in \CV_c$, we deliver a concatenation of smaller parts of its requested data available in the cache memory of other users in $\CV_c$, each with size $\binom{t_j}{t_c}$.


Next, for each state $s_j$, each file part $f^j_{\CV_j}$ is divided into $\binom{t_j}{t_c}$ smaller chunks.%, where $\mathcal{S}_u = \{s_{u_k}| \forall k \in \mathcal{K}\}$. 
Then, a sub-file $\hat{f}^{j}_{\CV}$ is created by concatenating a file chunk from each $\mathcal{V}_s$ such that $\mathcal{V} \subseteq \mathcal{V}_s$, where $\mathcal{V} \subseteq \mathcal{K}, |\mathcal{V}| = t_c$, i.e., $\hat{f}^{s}_{\mathcal{V}} = [NEW({f^{s}_{\mathcal{V}_s}})]_{\{\forall \mathcal{V}_s | \mathcal{V} \subseteq \mathcal{V}_s\}}$. Note that $|\mathcal{V}_s| \geq |\mathcal{V}|$, thus, there exist several $\mathcal{V} \subseteq \mathcal{V}_s$. Therefore, we use function $NEW(.)$ to make sure that unique file chunk is being dedicated to different subset $\mathcal{V}$ (see the example). Note that sub-file $\hat{f}^{s}_{\mathcal{V}}$ is available in the memory of all the users $k \in \mathcal{V}$.

For the delivery phase, $\binom{K}{t_c+1}$ transmission is required, where at each transmission $t_c+1$ users are being served with a common nested message. At each particular transmission, a nested message is transmitted to a subset of users, denoted as $\mathcal{D} \subseteq \mathcal{K}, |\mathcal{D}| = t_c+1$, as the following
\begin{equation}
    X_\mathcal{D} = *_{k \in \mathcal{D}} f^{s_{u_k}}_{\mathcal{D} \setminus k},
\end{equation}
where, $*$ is the nesting operation. Note that each user $k \in \mathcal{D}$ has all the sub-files $\{f^s_{\mathcal{V}}, \mathcal{V} \subset \mathcal{D}, |\mathcal{V}| = t_c\}$ but $f^{s_{u_k}}_{\mathcal{D} \setminus k}$, which must be transmitted with rate $r_{s_{u_k}}$. Thus, each user can cache out all the unwanted files in $X_\mathcal{D}$ with the help of its cache and decode its intended sub-file to recover the required file. Finally, the complete proposed cache placement and delivery scheme is summarised in algorithm~\ref{Alg_Main}.
\begin{theorem}
The proposed cache placement and delivery scheme satisfies all the users file requirement.
\begin{proof}
Consider user $k \in \mathcal{K}$ at state $s_{u_k}$, where it has $m_sF = \frac{t_{s_{u_k}} F}{K}$ [bits/Hz] available data in its cache and requires $f_{s_{u_k}} = F - m_{s_{u_k}}F = \frac{(K-t_{s_{u_k}})F}{K}$ remaining data from the transmitter. Based on the delivery scheme, each user receives $\binom{K-1}{t_c}$ sub-files $\{\hat{f}^{{s_{u_k}}}_{\mathcal{V}}, \mathcal{V} \subseteq \mathcal{K} \setminus k, |\mathcal{V}| = t_c$\} in the delivery phase. Each sub-file $\hat{f}^{{s_{u_k}}}_{\mathcal{V}}$ is the concatenated version of $\binom{K-t_c-1}{t_s-t_c}$ number of file-chunks with the size $\frac{F}{\binom{K}{t_s}\binom{t_{s_{u_k}}}{t_c}}$. As the result, $\frac{\binom{K-1}{t_c}\binom{K-t_c-1}{t_{s_{u_k}}-t_c}F}{\binom{K}{t_{s_{u_k}}}\binom{t_{s_{u_k}}}{t_c}}= \frac{(K-t_{s_{u_k}})F}{K}$ [bits/Hz] data is delivered through the transmitter and the remaining $\frac{t_{s_{u_k}}  F}{K}$ [bits/Hz] data is available in its cache.
\end{proof}
\end{theorem}
\subsection{Performance}
Though the placement and delivery scheme in this paper can be generalized, we use following assumptions for the performance analysis of the proposed method
\begin{itemize}
    \item The total available memory at each user is such that after solving~\eqref{cache-allocation} we have $m_s > 0, \forall s \in \mathcal{S}$.
    \item For each state $s \in \mathcal{S}$ we have integer $t_s = Km_s$, i.e., $t_s \in \{1,2, \dots, K\}$.
\end{itemize}
The generalized version of the cache placement and delivery scheme, along with the performance analysis is investigated in the simulation results (section~\ref{sec:simulation}).

\begin{lemma} \label{lemma:eqality}
At the optimal point the solution of~\eqref{cache-allocation} satisfies the following
\begin{equation} \label{eq:optimalms}
    \frac{F-m_sF}{r_s} = \frac{F-m_{s^{'}}F}{r_{s^{'}}}, \quad \forall \{s,s^{'}\} \in \mathcal{S}, s \neq s^{'}.
\end{equation}
    \begin{proof}
    The proof can be shown through contradiction. %Suppose at the optimally point there exist $s \in \mathcal{S}$ such that $\frac{F-m_s}{r_s} > \frac{F-m_{s^{'}}}{r_{s^{'}}}, \forall s^{'} \in \mathcal{S} \setminus s$, then by decreasing $m_s$ with $\delta$ and increasing the rest of states by $\frac{\delta}{|S|-1}$
    \end{proof}
\end{lemma}

\begin{lemma}\label{lemma:fs/rs}
At the optimal point the solution of~\eqref{cache-allocation} satisfies the following
\begin{equation} \label{eq: fs/rs}
    \frac{|f_s|}{r_s} = \frac{(S-M)F}{\sum\limits_{{s^{'}} \in \mathcal{S}}r_{s^{'}}}, \quad \forall s \in \mathcal{S}.
\end{equation}
where $|f_s| = F-m_sF$.
\begin{proof}
Since the total amount of available data for all the states is $SF$ and the total available cache dedicated to all the states at each user is $MF$, the sum of remaining data for all the states is
\begin{equation} \label{eq:sumfs}
    \sum\limits_{s \in \mathcal{S}}|f_s| = SF - MF.
\end{equation}
Now, using~\eqref{eq:optimalms} we have
\begin{equation} \label{eq:fsfsp}
    |f_s| = \frac{r_s}{r_{s^{'}}}|f_{s^{'}}|, \forall \{s, s^{'} \} \in \mathcal{S}.
\end{equation} 
Substituting~\eqref{eq:fsfsp} into~\eqref{eq:sumfs} and solving for $\frac{|f_{s^{'}}|}{r_{s^{'}}}$,~\eqref{eq: fs/rs} is achieved.
\end{proof}
\end{lemma}
Based on lemma~\ref{lemma:eqality} and lemma~\ref{lemma:fs/rs} the following statement holds.
\begin{theorem}\label{theorem:proposed transmission time}
the total delivery time of the proposed cache placement and delivery scheme is
\begin{equation}\label{eq:proposed transmission time}
    T_m = (\frac{K}{t_c + 1})\frac{(S-M)F}{\sum\limits_{s \in \mathcal{S}}r_s}.
\end{equation}
\begin{proof}
In general, each user $k \in \mathcal{K}$ at state $s_{u_k} \in \mathcal{S}$ requires $|f_{s_{u_k}}|$ [bits/Hz] to decode its intended data, which is delivered by $\binom{K-1}{t_c}$ transmissions (based on the proposed on the proposed delivery method). Since the transmitted data at each transmission has the same information, at each transmission $\frac{|f_{s_{u_k}}|}{\binom{K-1}{t_c}}$ [bits/Hz] with the rate $r_{s_{u_k}}$ [bits/Hz/s] is transmitted to user $k$. Thus, the total required time to serve user $k$ at each transmission is $\frac{1}{\binom{K-1}{t_c}}\frac{|f_{s_{u_k}}|}{r_{s_{u_k}}}$. Now, using~\eqref{eq: fs/rs} it can be deduced that each transmission takes exactly $\frac{1}{\binom{K-1}{t_c}}\frac{(S-M)F}{\sum\limits_{s \in \mathcal{S}}r_s}$ seconds. Using the fact that the total number of required transmissions to serve all the users is $\binom{K}{t_c + 1}$ and each transmission takes $\frac{1}{\binom{K-1}{t_c}}\frac{(S-M)F}{\sum\limits_{s \in \mathcal{S}}r_s}$ seconds, theorem~\ref{theorem:proposed transmission time} is proved.
\end{proof}
\end{theorem}
\begin{lemma}
The delivery time of the proposed delivery scheme satisfies the following statement
\begin{equation} \label{eq:tm/tu}
    \frac{T_m}{T_u} = \frac{1}{t_c+1}, \quad \forall s \in \mathcal{S}_u,
\end{equation}
where $T_u$ is the delivery time of unicasting.
\begin{proof}
In unicasting, only one user is served at each transmission. Thus, the total delivery time is $T_u = \sum\limits_{s \in \mathcal{S}_u}\frac{f_s}{r_s}$. Using~\eqref{eq: fs/rs}, the unicasting delivery time is $T_u = K\frac{(S-M)F}{\sum\limits_{s \in \mathcal{S}}r_s}$.
\end{proof}
\end{lemma}

\begin{corollary}
When users are in locations with low transmission rates, they can benefit from cache with higher $m_s$. As a result, $t_c$ will be larger, which will increase the proposed delivery gain and compensates for the low transmission rates.
\end{corollary}
\begin{theorem}
The proposed cache placement and delivery scheme has a bounded average delivery time gap from any optimal cache placement and delivery scheme. 
\begin{proof}
See arxiv.
\end{proof}
\end{theorem}


==> Uneven Cache Placement - ISIT _extend/Figures/Data/Fig23.tex <==
States	rates	Memory
1	3	25
2	2	50
3	1	75
4	2	50
5	3	25


==> Uneven Cache Placement - ISIT _extend/Figures/Data/Fig4.tex <==
K	Tu	Tx	Tm
2.00	22.417	13.0839	11.2092
4.00	44.834	14.5858	14.797
6.00	67.251	17.0666	14.394
8.00	89.668	17.6221	14.9472
10.00	112.085	19.5806	15.675
12.00	134.502	19.6288	15.8259
14.00	156.919	20.5986	15.8379
16.00	179.336	20.5849	16.1166
18.00	201.753	20.9576	16.2863
20.00	224.17	21.0379	16.5118
22.00	246.587	21.4939	16.3505
24.00	269.004	21.9699	16.5005
26.00	291.421	21.8099	16.6903
28.00	313.838	22.3583	16.6137
30.00	336.255	22.5763	16.5929
32.00	358.672	22.3293	16.8354
34.00	381.089	22.7776	16.9614
36.00	403.506	22.4904	16.6834
38.00	425.923	22.8297	16.8527
40.00	448.34	22.9195	17.032


==> Uneven Cache Placement - ISIT _extend/Figures/Data/Fig56.tex <==
M	Tu-Tm-S121	Tu-Tx-S121	Tu-Tm-S441	Tu-Tx-S441
0.0	1.00	1.00	1.00	1.00
0.1	1.125	1.715	1.1005	0.9352
0.2	1.4204	2.3821	1.2627	0.9259
0.3	1.8646	3.0289	1.4379	0.9054
0.4	2.5103	3.6647	1.5884	0.8623
0.5	3.7638	4.2871	1.8446	0.8065
0.6	5.2718	4.8986	2.06360	0.7465
0.7	6.5411	5.501	2.5547	0.6907
0.8	7.998	6.0954	3.1313	0.6663
0.9	8.996	6.6831	6.7314	0.7047


==> Uneven Cache Placement - ISIT _extend/Figures/Fig2.tex <==
%\begin{figure}
    \centering
    \resizebox{0.6\columnwidth}{!}{%

    \begin{tikzpicture}

    \begin{axis}
    [
    % put axis lines at left and bottom
    axis lines = left,
    % control axis labels
    xlabel near ticks,
    xlabel = \smaller {States},
    ylabel = \smaller {Rate [bits/Hz/s] \ref{rate}},
    ylabel near ticks,
    ymin = 0, %ymax = 20,
    % control legend position
    legend pos = north west,
    % control size of tick marks (10,20,30,etc)
    ticklabel style={font=\smaller},
    % control major grids
    grid=both,
    major grid style={line width=.2pt,draw=gray!30},
    % control minor grids
    %grid style={line width=.1pt, draw=gray!10},
    %minor tick num=5,
    %ybar interval=0.7,
    ]
    
    \addplot
    [mark = square, black]
    table[y=rates,x=States]{Figures/Data/Fig23.tex};
    %\addlegendentry{\tiny rate}
    \label{rate}
    \end{axis}
    
    \begin{axis}
    [
    % put axis lines at left and bottom
    axis lines = right,
    axis x line*=bottom,
    xtick={},
    xticklabels={},
    axis y line*=right,
    % control axis labels
    %xlabel near ticks,
    %xlabel = \smaller {States},
    ylabel = \smaller {Memory \%  \ref{memory}},
    ylabel near ticks,
    ymin = 0, ymax = 100,
    % control legend position
    %legend pos = north west,
    % control size of tick marks (10,20,30,etc)
    ticklabel style={font=\smaller},
    % control major grids
    %grid=both,
    major grid style={line width=.2pt,draw=gray!30},
    % control minor grids
    %grid style={line width=.1pt, draw=gray!10},
    %minor tick num=5,
    %ybar interval=0.7,
    ]
    
    \addplot
    [mark = x, gray]
    table[y=Memory,x=States]{Figures/Data/Fig23.tex};
    %\addlegendentry{\tiny memory}
    \label{memory}
    \end{axis}

    \end{tikzpicture}
    }

    \caption{Location-specific rate and memory distributions for Example~\ref{exmp:placement}.
    }
    \label{fig:rate&cache_distribution}
%\end{figure}

==> Uneven Cache Placement - ISIT _extend/Figures/Fig4.tex <==
%\begin{figure}
    \centering
    \resizebox{\columnwidth}{!}{%

    \begin{tikzpicture}

    \begin{axis}
    [
    % put axis lines at left and bottom
    axis lines = left,
    % control axis labels
    xlabel near ticks,
    xlabel = \smaller {The number of users ($K$)},
    ylabel = \smaller {Delivery time [ms]},
    ylabel near ticks,
    ymin = 0, %ymax = 20,
    % control legend position
    legend pos = north west,
    % control size of tick marks (10,20,30,etc)
    ticklabel style={font=\smaller},
    % control major grids
    grid=both,
    major grid style={line width=.2pt,draw=gray!30},
    % control minor grids
    %grid style={line width=.1pt, draw=gray!10},
    %minor tick num=5,
    %ybar interval=0.7,
    ]
    
    \addplot
    [mark = square, black]
    table[y=Tu,x=K]{Figures/Data/Fig4.tex};
    \addlegendentry{\tiny $T_u$}
    
    \addplot
    [mark = x, black!60]
    table[y=Tx,x=K]{Figures/Data/Fig4.tex};
    \addlegendentry{\tiny $T_x$}
    
    \addplot
    [dashed, black!40]
    table[y=Tm,x=K]{Figures/Data/Fig4.tex};
    \addlegendentry{\tiny $T_m$}
    
    \end{axis}

    \end{tikzpicture}
    }

    \caption{Average delivery time vs the user count~($K$), $M = \frac{3}{4}S$.
    }
    \label{fig:timegain_Kx}
%\end{figure}

==> Uneven Cache Placement - ISIT _extend/Figures/Fig5.tex <==
%\begin{figure}
    \centering
    \resizebox{\columnwidth}{!}{%

    \begin{tikzpicture}

    \begin{axis}
    [
    % put axis lines at left and bottom
    axis lines = left,
    % control axis labels
    xlabel near ticks,
    xlabel = \smaller {M [Data Units]},
    ylabel = \smaller {Performance Ratio},
    ylabel near ticks,
    ymin = 0, %ymax = 20,
    % control legend position
    legend pos = north west,
    % control size of tick marks (10,20,30,etc)
    ticklabel style={font=\smaller},
    % control major grids
    grid=both,
    major grid style={line width=.2pt,draw=gray!30},
    % control minor grids
    %grid style={line width=.1pt, draw=gray!10},
    %minor tick num=5,
    %ybar interval=0.7,
    ]
    
    \addplot
    [mark = x, black]
    table[y=Tu-Tx-S121,x=M]{Figures/Data/Fig56.tex};
    \addlegendentry{\tiny $\frac{T_u}{T_x}$}
    
    \addplot
    [mark = square, black!60]
    table[y=Tu-Tm-S121,x=M]{Figures/Data/Fig56.tex};
    \addlegendentry{\tiny $\frac{T_u}{T_m}$}
    
    \end{axis}

    \end{tikzpicture}
    }

    \caption{Relative gain in delivery time vs the cache size~($M$), $K = 10$, $S = 121$.
    }
    \label{fig:time_Mxs121}
%\end{figure}

==> Uneven Cache Placement - ISIT _extend/Figures/Fig6.tex <==
%\begin{figure}
    \centering
    \resizebox{\columnwidth}{!}{%

    \begin{tikzpicture}

    \begin{axis}
    [
    % put axis lines at left and bottom
    axis lines = left,
    % control axis labels
    xlabel near ticks,
    xlabel = \smaller {M [Data Units]},
    ylabel = \smaller {Performance Ratio},
    ylabel near ticks,
    ymin = 0, %ymax = 20,
    % control legend position
    legend pos = north west,
    % control size of tick marks (10,20,30,etc)
    ticklabel style={font=\smaller},
    % control major grids
    grid=both,
    major grid style={line width=.2pt,draw=gray!30},
    % control minor grids
    %grid style={line width=.1pt, draw=gray!10},
    %minor tick num=5,
    %ybar interval=0.7,
    ]
    
    \addplot
    [mark = x, black]
    table[y=Tu-Tx-S441,x=M]{Figures/Data/Fig56.tex};
    \addlegendentry{\tiny $\frac{T_u}{T_x}$}
    
    \addplot
    [mark = square, black!60]
    table[y=Tu-Tm-S441,x=M]{Figures/Data/Fig56.tex};
    \addlegendentry{\tiny $\frac{T_u}{T_m}$}
    
    \end{axis}

    \end{tikzpicture}
    }

    \caption{Relative gain in delivery time vs the cache size~($M$), $K = 10$, $S = 441$.
    }
    \label{fig:timegain_Mx441}
%\end{figure}

==> Uneven Cache Placement - ISIT _extend/Figures/Fig_mem.tex <==
%\begin{figure}
    \centering
    \resizebox{\columnwidth}{!}{%

    \begin{tikzpicture}

    \begin{axis}
    [
    % put axis lines at left and bottom
    axis lines = left,
    % control axis labels
    xlabel near ticks,
    xlabel = \smaller {States},
    ylabel = \smaller {\% memory},
    ylabel near ticks,
    ymin = 0, %ymax = 20,
    % control legend position
    %legend pos = north west,
    % control size of tick marks (10,20,30,etc)
    ticklabel style={font=\smaller},
    % control major grids
    grid=both,
    major grid style={line width=.2pt,draw=gray!30},
    % control minor grids
    %grid style={line width=.1pt, draw=gray!10},
    %minor tick num=5,
    %ybar interval=0.7,
    ]
    
    \addplot
    [mark = square, black]
    table[y=Memory,x=States]{Figures/Data/Fig23.tex};
    %\addlegendentry{\tiny $T_u$}
    
    \end{axis}

    \end{tikzpicture}
    }

    \caption{Location-specific memory distribution.
    }
    \label{fig:cache_distribution}
%\end{figure}

==> Uneven Cache Placement - ISIT _extend/Intro.tex <==
The current dominant interface for human-computer interaction is through mobile flat-screen devices such as smartphones and tablets. The next interface evolution is expected to bring forward wireless immersive viewing experiences facilitated by more capable wearable gadgets submerging users into the three-dimensional~(3D) digital world. However, such an evolution requires powerful and agile external radio connections. It imposes extremely stringent key performance indicators (KPIs) that are simply beyond what is possible with the current networking standards~\cite{han2017problem}. This necessitates new techniques that leverage recent advances in communication, storage, computing, big data analysis and machine learning~\cite{bastug2017toward}.

In this regard, using cheap on-device storage for improving bandwidth efficiency is considered a promising technique~\cite{bastug2014living}. In~\cite{sun2019communications}, it is shown that utilizing caching and computing capabilities of mobile VR devices effectively alleviates the traffic burden over the wireless network.
In~\cite{maddah2014fundamental}, a new caching technique known as \emph{Coded Caching (CC)} is introduced. In CC, well-defined fragments of all the files in the library are stored in the cache memories, creating a cache-aided multicasting gain during the delivery phase and resulting in a \emph{global caching gain}.
%
%Instead of locally caching entire files at the end-user as in~\cite{sun2019communications}, \emph{coded caching} (CC) proposed in~\cite{maddah2014fundamental}, allows storing fragments of all files in the library in the users' cache memories. As a result, multicasting opportunities are provided in the delivery phase, which results in a \emph{global caching gain}~\cite{maddah2014fundamental}.
%
The original CC scheme in~\cite{maddah2014fundamental} is extended to multi-server networks in~\cite{shariatpanahi2016multi}, and later to wireless multi-antenna systems in~\cite{shariatpanahi2018multi,tolli2017multi}. A device-to-device (D2D) extension of multi-antenna coded caching is also investigated in~\cite{mahmoodi2020d2d}. Meantime, various practical limitations of coded caching have been addressed by the research community. Most notably, the large subpacketization requirement, defined as the number of smaller parts each file should be split into, is addressed in~\cite{lampiris2018adding,salehi2020lowcomplexity}, while the effect of the subpacketization on the low-SNR rate is investigated in~\cite{salehi2019subpacketization}.

A less-studied problem of coded caching schemes, affecting content delivery applications in general and immersive viewing applications in particular, is the \textit{near-far} issue. Due to the underlying multicasting nature of coded caching schemes, the achievable rate in any multicast message is limited to the rate of the user with the worst channel conditions. In~\cite{destounis2020adaptive}, a congestion control technique is proposed to avoid serving users in adverse fading conditions, while in~\cite{salehi2020coded} multiple descriptor codes~(MDC) are utilized to serve ill-conditioned users with a lower quality-of-experience. Unlike~\cite{destounis2020adaptive,salehi2020coded}, which are based on traditional XOR-ing of data elements, in~\cite{tang2017coded} nested code modulation (NCM) is proposed to allow building codewords that serve every user in the multicasting group with a different rate. This multi-rate property is achieved by altering the modulation constellation using side information on the file library and other users' requests.
%is possible by benefiting from \textit{prior information}, i.e., the requested data of the other receivers, at each receiver~\cite{tang2011full}. 
A similar multi-rate transmission scheme can also be found in~\cite{chen2010novel}. However, the aforementioned approaches are not suitable for dynamic real-time applications, where users frequently move inside the network, and their achievable rate changes accordingly.

This paper introduces a new location-dependent coded caching scheme for efficient content delivery in wireless access networks. We consider a wireless communication scenario in which the users are free to move, and their requested content depends on their current location. Furthermore, the requested content at each location is assumed to be of the same size. As a specific use-case, we assume a multi-user immersive viewing environment where a group of users is submerged into a network-based immersive application that runs on a high-end eye-wear. Such a use-case necessitates heavy multimedia traffic and guaranteed user quality of experience (QoE) throughout the operating environment. In this regard, a location-dependent, uneven memory allocation is carried out based on the attainable data rate at each given location. Moreover, a novel multicast transmission scheme with an underlying NCM structure to support different data rates is devised to deliver the missing user-specific content within the same multicast transmission. Due to the optimized location-dependent cache placement, the worst-case delivery time is minimized across all the locations.


%As a result, the efficient multicasting of codewords at any time instant results in the reduction of the total delivery time compared to the unicasting scenario. %which depends on the total cache size in the network and the users' proximity to each other. 
%The outcome is a non-symmetric location-dependent scheme, allowing efficient usage of coded caching techniques especially for future immersive viewing setups.

%The rest of the paper is organized as follows. In Section~\ref{section:system_model} we propose the considered system model. The new location-dependent coded caching scheme is presented in Section~\ref{section:the_new_scheme} and its performance is discussed in Section~\ref{section:performance}. In Section~\ref{section:sim_results}, we analyze the performance of the proposed scheme with numerical simulations. Finally, in Section~\ref{section:conclusion} we conclude the paper and propose future research directions. Throughout the paper, we have used calligraphic upper-case letters for denoting sets. Other notations are clarified when they are used in the text.

%An increasingly large portion of today's population is continuously connected to the virtual information world through mobile flat-screen devices, such as smartphones and tablets. The next step in the evolution of human-computer interfaces will bring forward immersive viewing experience facilitated by more capable wearable gadgets that submerge users to the three-dimensional (3D) digital world. %Although the idea of digital immersion has been around for decades [...], its mass adoption was severely hampered by movement-restricting wired connections between the interfacing headsets and the external hardware. However, since 2018, a whole new generation of powerful and affordable untethered headsets has flooded the market.
%
%These emerging wireless immersive viewing applications require powerful and agile external radio connections and impose stringent communication requirements that include extremely high throughput links to the processing unit (e.g., up to 3.3 Gbps for ultimate 3D video) and ultra-low over-the-air latencies as low as 1 ms [...,...]. %Failure to satisfy these requirements leads to so-called cybersickness, which manifests as discomfort, disorientation or nausea caused by human sensory conflict [...]. These constraining features of human perception result in much higher importance of the radio link reliability and stability for peak data rates than in the case of traditional 2D screens. 

%These requirements are beyond what's possible with current networking standards [mehddi-2017-CMAG]. As a result, new techniques which leverage recent advances in storage/memory, communication/connectivity, computing, big data analytics, artificial intelligence (AI), machine vision, and others are required [mehddi-2017-CMAG]. 

%One key solution to this problem lies in the efficient utilization of the ever cheap in-device memories [mehddi-2014-CMAG]. Authors in [immers-caching-2D-fov-2018, immers-caching-3D-fov-2019] have shown that utilizing caching and computing capabilities of mobile VR devices alleviate the traffic burden over wireless network significantly. \textbf{Linking statement to the next paragraph is requiered}%via multipoint coded caching (CC) [...].

%Different from traditional caching methods which tend to store the data files completely, novel cache placement method known as \textit{coded caching} (CC) has been proposed in [maddah-2014]. %In this approach, parts of all the files are carefully stored in the cache of all the users, which later on creates multicasting opportunities. 
%Benefiting from cache memory of all the users in the network (memory pool), CC enjoys so-called \textit{global caching} gain in its transmission mechanism.

%CC, initially considered for wired networks, has also shown promising performance in increasing the wireless network's spectrum efficiency [pooya multi server, antti-TWC-2020, H.B.M-arxive-2020]. To benefit from the CC gain in a wireless environment, many works have attempted to tailor the scheme for the wireless degraded nature. For instance, \textit{sub-packetization} issue of the proposed CC scheme for the wireless notwork has been addressed in [Mohammad, petros] \textbf{Mohammad can describe this issue properly}. Another crucial issue in the CC wireless setting, known as \emph{near-far} problem, is that the rate for the common message is always limited by the worst user. Since users typically experience different link conditions in real-life scenarios, traditional CC implementation in a wireless network is not well suited. To tackle the issue, while the authors in~\cite{Alpha_fair_CC} propose a congestion control technique to avoid serving users in a fading state, authors in~\cite{UOS_for_CC} benefit from a threshold-based scheduling approach to eliminate the users below the threshold and serve the rest of the users. 

%The traditional CC approach generates the downlink (DL) message, intended for a group of users, by XORing several data. As a result, the message must be transmitted with the weakest intended user's rate so that all the group members can decode it~\cite{Alpha_fair_CC, UOS_for_CC}. Different from the traditional approach, [Tang] benefits from \textit{nested code modulation} (NCM) along with heterogeneous cache size allocation to achieve the sum-rate performance without being limited to the ill-conditioned users. 
%NCM is a novel multicasting technique originally introduced in a two-way relaying network, which supports different link rates with a single transmission~\cite{NCM-2011}. 
%This is done by benefiting from \textit{a priory information} at the transceivers. Similar idea has been proposed in a two-user two-way relaying network, where the transmitter adopts a joint coded modulation (JCM) technique to modulate two intended data simultaneously~\cite{JCM/relaying-2013-Chen}. Unlike~\cite{JCM/constellation-expansion}, which expands the constellation size for jointly coded data modulation \textcolor{red}{this one is also called JCM}, authors in~\cite{JCM/relaying-2013-Chen} benefit from a novel relabeling technique. Therefore, benefiting from \textit{a priory information}, each user demodulates the received data using different constellation sizes. As a result, different users can be supported with different rates by a single transmission.

%Multi-user multiple-input-single-output (MU-MISO) setup has been considered in [soheil], where each user is served at the rate of its channel through unequal cache placement. In this approach, users with the lowest available rate are mostly served by more extensive available data in their caches. As a result, less wireless resources are dedicated to users with the poor channel, which compensates for the \emph{near-far} problem. 

%A novel multicasting technique has been introduced in a two-user two-way relaying network, supporting different link rates without any performance loss~\cite{JCM/relaying-2013-Chen}. In this technique, benefiting from \textit{a priory information} available at the transceivers, the transmitter adopts a joint coded modulation (JCM) technique to modulate two intended data simultaneously. Unlike~\cite{JCM/constellation-expansion}, which expands the constellation size for jointly coded data modulation \textcolor{red}{this one is also called JCM}, authors in~\cite{JCM/relaying-2013-Chen} benefit from a novel relabeling technique. Therefore, benefiting from \textit{a priory information}, each user demodulates the received data using different constellation sizes. As a result, different users can be supported with different rates by a single transmission.

%Having the same idea as in~\cite{JCM/relaying-2013-Chen}, authors in~\cite{NCM-2011} propose a novel modulation technique that supports several users with different link rates with a single transmission. The proposed method in~\cite{NCM-2011} ideally achieves all the users' link full rate.  Authors in~\cite{CC-unequal-link-rate-2018} have shown that all the users' link capacity can be ideally achieved in a wireless CC network by benefiting from the NCM technique.

%However, the approach proposed in [them] is not suitable for access applications, where users move frequently inside the network and their achievable rate also changes accordingly. Motivated by this fact, in this paper we consider a location-base cache placement and delivery scheme, where users rate changes at each time-slot based on their relative position to the access point. A perfect match for the considered scenario is multi-user immersive viewing application, where users are allowed to move freely inside the network. 

%We envision an XR or hyper-reality environment (educational, industrial, gaming, defense, social networking, etc.), where a large group of users is submerged into a network-based immersive application that runs on a high-end eye-wear and, hence, requires heavy multimedia traffic and is bound to guarantee a required level of user quality of experience (QoE) throughout the operating theatre. All this multimedia content eventually rendered to be seen by the participants is user-specific and requires extremely fast updates with delays lower than the human perception thresholds. Notably, a large part of rich multimedia content for rendering a certain viewpoint is common among the users, which offers opportunities for efficient use of pooled memory resources through intelligent cache placement and network coded multicast content delivery mechanisms.

%Though cache placement and delivery in this context is considered before, most of the case study consider a single VR device for their proposed schemes [immers-caching-2D-fov-2018, immers-caching-3D-fov-2018]. Considering the promising achievements of the cc network investigated in [Tang], we extend the study case to the access network with special focus on the immersive viewing application. We show that the proposed cache placement and delivery scheme significantly improves the network performance specially for critical scenarios, where most of the users are located in ill-conditioned locations.

%\textcolor{red}{Network traffic} has increased unprecedentedly in the recent few years due to advent of new services, such as high-definition on-demand video streaming and mobile virtual realities. \textbf{THE FIRST TWO PARAGRAPHS BORROWED FROM ANTTI'S PROPOSAL CAN BE SUMMARIZED FOR HERE}
 
%one key enabler to handle such services is moving the data closer to the end-user in order to decrease the load on wireless network. \textbf{ARE WE TALKING ABOUT EDGE CACHING? IF YES, IT WOULD BE NICE TO INCLUDE SOME REFERENCES AND ADD A FEW MOTIVATING SENTENCES, LIKE IT HAS HELPED TO ...}
 
%CC, initially considered for wired network, has shown promising performance in increasing the spectrum efficiency. \textbf{CC SHOULD BE LINKED TO EDGE CACHING CAREFULLY. THE RELATION BETWEEN THIS PARAGRAPH AND THE PREVIOUS ONE SHOULD BE WRITTEN NICELY. ALSO, I DON'T GET WHAT YOU MEAN BY "INITIALLY CONSIDERED FOR WIRELESS NETWORK"?}
  
%In order to benefit from the CC gain in wireless network many works have attempted to tailor the scheme for the wireless degraded nature. \textbf{PUT REFERENCES, WITH A VERY BRIEF TIMELINE. E.G., CODED CACHING IS FIRST EXTENDED TO WIRELESS NETWORKS IN ... AND THEN IN ... THE PERFORMANCE IS IMPROVED BY USING OPTIMIZED BEAMFORMERS}
  
%Main bottleneck of the conventional cc approach proposed by []-[] is that the performance gain is highly affected by the weakest user. \textbf{THIS PARAGRAPH IS A NICE PLACE FOR CITING SOME OF OUR OWN WORKS. E.G., CC ISSUES IN WIRELESS NETWORKS, SUCH AS SUBPACKETIZATION AND A POSSIBLE EXTENSION TO D2D SETUPS HAVE BEEN STUDIED EXTENSIVELY. ONE OTHER IMPORTANT ISSUE IS THE NEAR-FAR PROBLEM, WHICH MEANS...}

%\textbf{THE FOLLOWING PARAGRAPHS NEED TO BE POLISHED.} In order to alleviate the degraded nature of the wireless network, unequal cache placement is proposed in [soheil], where the user with lowest available rate is mostly served by the larger available data in its cache.
 
%similar idea has also been adopted in [Tang], by benefiting from nested code modulation along with heterogeneous cache size allocation, Where they were able to achieve the sum-rate performance without being limited to the worst user.
 

%\textbf{IF WE START THE INTRO BY IMMERSIVE VIEWING, WE SHOULD BE MORE CAREFUL HERE.} 
%A perfect match for the considered scenario is multi-user immersive viewing application, where users are allowed to move freely inside the network. Though cache placement and delivery in this context is considered before, most of the case study consider a single VR device for their proposed schemes [immers-caching-2D-fov-2018, immers-caching-3D-fov-2018]. 

%\textbf{WE NEED MORE DESCRIPTION OF OUR KEY IDEA AND RESULTS.}
%Though cache placement and delivery in this context is considered before, most of the case study consider a single VR device for their proposed schemes.


%\begin{itemize}
%     \item Immersive viewing is an important application for future networks.
%    \item The market size is also expected to grow.
%    \item Currently deployed application are mostly wired.
%    \item A true immersive viewing application has to be wireless.
%    \item It has applications in many fields: gaming, medicine, industry, education, etc.
%    \item Wireless connectivity means dynamic conditions of the network: users are free to move.
%    \item It also means the need for very high throughput together with controlled delay.
%    \item The required throughput is beyond what's possible with current networking standards.
%    \item We need new techniques to cope with the requirements.
%    \item Using caching (in general) is an appropriate approach, considering the declining price of the memory chips.
%    \item It is also interesting in our case as the application is based on video-streams, from which an important part is static.
%    \item Coded caching elevates the performance of traditional caching by making use of memory pools.
%    \item This is again nicely applicable to our scenario as there are nearby users forming memory pools.
%    \item Of course, there are important issues to be addressed before a practical implementation.
%\end{itemize}

%We can get help with the Nokia application.

%Enhance the figure: put more details maybe.

%Justify the state-based model in the intro.

%Talk more about the FoV and interpolation between the FoV of the states. Make some Googling about the software structure and what can be cached. The reference scenario is to do all the computation in the edge. We want to say that we can pre-compute part of the rendering and put it in the cache memories.

%Maybe Mehdi paper can be a good starting point.

%Or Nokia 3D camera.

%Check if the data really can be split into static and dynamic parts. And the static part is the huge part and can be cached. And we are just focusing on the static part.

%Make sure using NCM as is done in this paper is correct.


%The rest of the paper is organized as follows. In Section~\ref{section:system_model} we propose the considered system model. The new location-dependent coded caching scheme is presented in Section~\ref{section:the_new_scheme} and its performance is discussed in Section~\ref{section:performance}. In Section~\ref{section:sim_results}, we analyze the performance of the proposed scheme with numerical simulations. Finally, in Section~\ref{section:conclusion} we conclude the paper and propose future research directions. Throughout the paper, we have used calligraphic upper-case letters for denoting sets. Other notations are clarified when they are used in the text.



==> Uneven Cache Placement - ISIT _extend/LiteratureRev.tex <==
Sample citation~\cite{maddah2014fundamental}.

\begin{itemize}
    \item Coded caching
    \item Wireless coded caching
    \item Coded caching with uneven cache placement (?)
    \item Caching applications in immersive viewing
\end{itemize}

==> Uneven Cache Placement - ISIT _extend/MyCommands.tex <==
\newtheorem{thm}{Theorem}
\newtheorem{lem}{Lemma}%[section]
\newtheorem{prop}[thm]{Proposition}
\newtheorem{cor}{Corollary}
\newtheorem{conj}{Conjecture}[section]
\newtheorem{exmp}{Example}%[section]
\theoremstyle{definition}
\newtheorem{defn}{Definition}[section]
\newtheorem{rem}{Remark}

% Calligraphic Letters
\newcommand{\CA}[0]{{\mathcal{A}}}
\newcommand{\CB}[0]{{\mathcal{B}}}
\newcommand{\CC}[0]{{\mathcal{C}}}
\newcommand{\CD}[0]{{\mathcal{D}}}
\newcommand{\CE}[0]{{\mathcal{E}}}
\newcommand{\CF}[0]{{\mathcal{F}}}
\newcommand{\CG}[0]{{\mathcal{G}}}
\newcommand{\CH}[0]{{\mathcal{H}}}
\newcommand{\CI}[0]{{\mathcal{I}}}
\newcommand{\CJ}[0]{{\mathcal{J}}}
\newcommand{\CK}[0]{{\mathcal{K}}}
\newcommand{\CL}[0]{{\mathcal{L}}}
\newcommand{\CM}[0]{{\mathcal{M}}}
\newcommand{\CN}[0]{{\mathcal{N}}}
\newcommand{\CO}[0]{{\mathcal{O}}}
\newcommand{\CP}[0]{{\mathcal{P}}}
\newcommand{\CQ}[0]{{\mathcal{Q}}}
\newcommand{\CR}[0]{{\mathcal{R}}}
\newcommand{\CS}[0]{{\mathcal{S}}}
\newcommand{\CT}[0]{{\mathcal{T}}}
\newcommand{\CU}[0]{{\mathcal{U}}}
\newcommand{\CV}[0]{{\mathcal{V}}}
\newcommand{\CW}[0]{{\mathcal{W}}}
\newcommand{\CX}[0]{{\mathcal{X}}}
\newcommand{\CY}[0]{{\mathcal{Y}}}
\newcommand{\CZ}[0]{{\mathcal{Z}}}

% Boldface Letters
\newcommand{\Ba}[0]{{\mathbf{a}}}
\newcommand{\Bb}[0]{{\mathbf{b}}}
\newcommand{\Bc}[0]{{\mathbf{c}}}
\newcommand{\Bd}[0]{{\mathbf{d}}}
\newcommand{\Be}[0]{{\mathbf{e}}}
\newcommand{\Bf}[0]{{\mathbf{f}}}
\newcommand{\Bg}[0]{{\mathbf{g}}}
\newcommand{\Bh}[0]{{\mathbf{h}}}
\newcommand{\Bi}[0]{{\mathbf{i}}}
\newcommand{\Bj}[0]{{\mathbf{j}}}
\newcommand{\Bk}[0]{{\mathbf{k}}}
\newcommand{\Bl}[0]{{\mathbf{l}}}
\newcommand{\Bm}[0]{{\mathbf{m}}}
\newcommand{\Bn}[0]{{\mathbf{n}}}
\newcommand{\Bo}[0]{{\mathbf{o}}}
\newcommand{\Bp}[0]{{\mathbf{p}}}
\newcommand{\Bq}[0]{{\mathbf{q}}}
\newcommand{\Br}[0]{{\mathbf{r}}}
\newcommand{\Bs}[0]{{\mathbf{s}}}
\newcommand{\Bt}[0]{{\mathbf{t}}}
\newcommand{\Bu}[0]{{\mathbf{u}}}
\newcommand{\Bv}[0]{{\mathbf{v}}}
\newcommand{\Bw}[0]{{\mathbf{w}}}
\newcommand{\Bx}[0]{{\mathbf{x}}}
\newcommand{\By}[0]{{\mathbf{y}}}
\newcommand{\Bz}[0]{{\mathbf{z}}}

\newcommand{\BA}[0]{{\mathbf{A}}}
\newcommand{\BB}[0]{{\mathbf{B}}}
\newcommand{\BC}[0]{{\mathbf{C}}}
\newcommand{\BD}[0]{{\mathbf{D}}}
\newcommand{\BE}[0]{{\mathbf{E}}}
\newcommand{\BF}[0]{{\mathbf{F}}}
\newcommand{\BG}[0]{{\mathbf{G}}}
\newcommand{\BH}[0]{{\mathbf{H}}}
\newcommand{\BI}[0]{{\mathbf{I}}}
\newcommand{\BJ}[0]{{\mathbf{J}}}
\newcommand{\BK}[0]{{\mathbf{K}}}
\newcommand{\BL}[0]{{\mathbf{L}}}
\newcommand{\BM}[0]{{\mathbf{M}}}
\newcommand{\BN}[0]{{\mathbf{N}}}
\newcommand{\BO}[0]{{\mathbf{O}}}
\newcommand{\BP}[0]{{\mathbf{P}}}
\newcommand{\BQ}[0]{{\mathbf{Q}}}
\newcommand{\BR}[0]{{\mathbf{R}}}
\newcommand{\BS}[0]{{\mathbf{S}}}
\newcommand{\BT}[0]{{\mathbf{T}}}
\newcommand{\BU}[0]{{\mathbf{U}}}
\newcommand{\BV}[0]{{\mathbf{V}}}
\newcommand{\BW}[0]{{\mathbf{W}}}
\newcommand{\BX}[0]{{\mathbf{X}}}
\newcommand{\BY}[0]{{\mathbf{Y}}}
\newcommand{\BZ}[0]{{\mathbf{Z}}}

% Serif Letters
\newcommand{\Sfa}[0]{{\mathsf{a}}}
\newcommand{\Sfb}[0]{{\mathsf{b}}}
\newcommand{\Sfc}[0]{{\mathsf{c}}}
\newcommand{\Sfd}[0]{{\mathsf{d}}}
\newcommand{\Sfe}[0]{{\mathsf{e}}}
\newcommand{\Sff}[0]{{\mathsf{f}}}
\newcommand{\Sfg}[0]{{\mathsf{g}}}
\newcommand{\Sfh}[0]{{\mathsf{h}}}
\newcommand{\Sfi}[0]{{\mathsf{i}}}
\newcommand{\Sfj}[0]{{\mathsf{j}}}
\newcommand{\Sfk}[0]{{\mathsf{k}}}
\newcommand{\Sfl}[0]{{\mathsf{l}}}
\newcommand{\Sfm}[0]{{\mathsf{m}}}
\newcommand{\Sfn}[0]{{\mathsf{n}}}
\newcommand{\Sfo}[0]{{\mathsf{o}}}
\newcommand{\Sfp}[0]{{\mathsf{p}}}
\newcommand{\Sfq}[0]{{\mathsf{q}}}
\newcommand{\Sfr}[0]{{\mathsf{r}}}
\newcommand{\Sfs}[0]{{\mathsf{s}}}
\newcommand{\Sft}[0]{{\mathsf{t}}}
\newcommand{\Sfu}[0]{{\mathsf{u}}}
\newcommand{\Sfv}[0]{{\mathsf{v}}}
\newcommand{\Sfw}[0]{{\mathsf{w}}}
\newcommand{\Sfx}[0]{{\mathsf{x}}}
\newcommand{\Sfy}[0]{{\mathsf{y}}}
\newcommand{\Sfz}[0]{{\mathsf{z}}}

\newcommand{\SfA}[0]{{\mathsf{A}}}
\newcommand{\SfB}[0]{{\mathsf{B}}}
\newcommand{\SfC}[0]{{\mathsf{C}}}
\newcommand{\SfD}[0]{{\mathsf{D}}}
\newcommand{\SfE}[0]{{\mathsf{E}}}
\newcommand{\SfF}[0]{{\mathsf{F}}}
\newcommand{\SfG}[0]{{\mathsf{G}}}
\newcommand{\SfH}[0]{{\mathsf{H}}}
\newcommand{\SfI}[0]{{\mathsf{I}}}
\newcommand{\SfJ}[0]{{\mathsf{J}}}
\newcommand{\SfK}[0]{{\mathsf{K}}}
\newcommand{\SfL}[0]{{\mathsf{L}}}
\newcommand{\SfM}[0]{{\mathsf{M}}}
\newcommand{\SfN}[0]{{\mathsf{N}}}
\newcommand{\SfO}[0]{{\mathsf{O}}}
\newcommand{\SfP}[0]{{\mathsf{P}}}
\newcommand{\SfQ}[0]{{\mathsf{Q}}}
\newcommand{\SfR}[0]{{\mathsf{R}}}
\newcommand{\SfS}[0]{{\mathsf{S}}}
\newcommand{\SfT}[0]{{\mathsf{T}}}
\newcommand{\SfU}[0]{{\mathsf{U}}}
\newcommand{\SfV}[0]{{\mathsf{V}}}
\newcommand{\SfW}[0]{{\mathsf{W}}}
\newcommand{\SfX}[0]{{\mathsf{X}}}
\newcommand{\SfY}[0]{{\mathsf{Y}}}
\newcommand{\SfZ}[0]{{\mathsf{Z}}}

%=====================================================================================================================================
% ===========================================================================
% File Name: commands.tex
% File Creation Date: 15.6.1995
% Author: Markku Juntti
% Description: Includes useful commands for Latex edition.
% ===========================================================================

\renewcommand{\Re}{\mbox{Re}}
\renewcommand{\Im}{\mbox{Im}}

% Bold-face Greek letters
\renewcommand{\vec}[1]{\bf{#1}}     %equation styles %vector/matrix


==> Uneven Cache Placement - ISIT _extend/NewScheme.tex <==
Similar to other coded caching schemes in the literature, our new NCM-based scheme also works in two distinct phases, cache placement and content delivery. For better clarification, throughout the discussions we frequently refer to the example network considered in Section~\ref{section:example_net}.
%However, the cache placement phase itself is performed in two steps: memory allocation and pool arrangement.

%The NCM-based cache placement is performed in two sub-phases: location-based cache portion allocation and cache pool arrangement. For the first phase, based on each specific location rate, we aim to minimize the maximum delivery time for all the states. In this manner, we aim to provide the minimum achievable delivery time for each state based on the fact that all the states have the same access probability. 

\subsection{Cache Placement}
For cache placement, we first determine the amount of cache memory (at every user) allocated to storing $F^i$, where $F^i$ is the file required for the user $u_i$ located at state $s_i$, $i \in \CS$. During this memory allocation process, we aim to minimize the maximum delivery time for all the states, assuming that all the states have the same access probability. From the system model, we know that the size of each $F^i$ is $F$ data units, and hence, if every user $u_j$ dedicates $m_iF$ data units in its cache memory for storing $F^i$, $F-m_iF$ data units should be delivered over the communication channel. As the result, if the single-user achievable rate at state $s_i$ is equal to $r_i$, the total delivery time for this state is $T_i = \frac{F-m_iF}{r_i}$. Finally, memory allocation for minimizing the maximum delivery time can be found by solving the following linear programming problem

%In general, at the state $s \in \mathcal{S}$ the total amount of $F_s$ [bits/Hz/s] needs to be delivered for the users located in this state. Since each user $k$ dedicates $m_s$ portion of its memory to cache some portion of the required data for this location, $F_s - m_s$ remaining data must be delivered to the user $k$ in state $s$ with available rate $r_s$. Therefore, the total required time to serve a user at state $s$ is $T_s = \frac{F_s - m_s}{r_s}$. Since all the states have the same access probability, there is no priority for any state. In this regard, we aim to allocate the memory portion to states such that the maximum delivery time among all the states is minimized. Note that each user has a limited memory of size $MF$ [bits/Hz]. Therefore, the memory allocation problem can be formulated to a LP as follows

\begin{equation}
\begin{aligned}
\label{cache-allocation}
 \text{LP} \ : \quad &\min_{\{m_i\}, \gamma}  \gamma\\
&\textrm{s.t.} \quad  \frac{F-m_iF}{r_i} \leq \gamma, \ \forall i \in \CS, \\
& \sum_{i \in \CS} m_i = M,\\
& m_i \geq 0, \ \forall i \in \CS, \\
& \gamma \geq 0.
\end{aligned}
\end{equation}

By solving~\eqref{cache-allocation}, the amount of cache memory (at every user) dedicated to each state is determined. Next, we arrange all the users' memory based on cache placement proposed in~\cite{maddah2014fundamental}. Note that in our proposed method, required files in each state are considered as a separate library, and the algorithm in~\cite{maddah2014fundamental} is performed for each state independent of the other states.
%\subsection{Cache Placement}
%Cache placement for each state follows the original coded caching scheme proposed in~\cite{maddah2014fundamental}. 
In this regard, $F^i$ is partitioned into $\binom{K}{t_i}$ parts denoted by $f^{i}_{\CV_i}$, where $\CV_i$ denotes a subset of users with $|\CV_i| = t_i$, and $t_i = Km_i$. Then, every user $k \in \CK$ fills up its cache as
\begin{equation}
    \CZ_k = \{f^{i}_{\CV_i} | \ \forall i, \forall \CV_i \ni k \} \; .
\end{equation}
%with some parts from all the states such that $\mathcal{Z}_k = \{f^{s}_{\CV} | \ \forall \CV, \  k \in \CV, \forall s\}$.

It can be easily verified that this cache placement satisfies the memory constraints. This is due to the fact that 
%\begin{theorem}
%The proposed cache placement satisfies the memory constraint.
%\begin{proof}
at each state $s_i$ the required file $F^i$ is divided into $\binom{K}{t_i}$ parts. Each user $k \in \CK$ stores $\binom{K-1}{t_i-1}$ of these parts, and hence, the total memory dedicated to state $s_i$ is
\begin{equation}
    \frac{\binom{K-1}{t_i-1}F^i}{\binom{K}{t_i}}=\frac{t_i F^i}{K} \; .
\end{equation}
data bits. Now, replacing $t_i$ with $K m_i$ and summing over all the states, we get $\sum_{s_i \in \CS}m_i F^i = MF$.
%\end{proof}
%\end{theorem}

\begin{algorithm}
	\caption{Location-based Cache Placement\label{Alg_Main}}
	\begin{algorithmic}[1]
		
%		\Procedure{MEM\_ALLOC}%{$\{ F^i, r_i ; \forall s_i \in \CS \}$}
		
%		\State $\mathcal{M} =  \arg\min\limits_{\CM = \{m_i\}}\max\limits_{i} \frac{F^i-m_i}{r_i} $
		%= \left\{m_{s_i} \bigg| \frac{F_s-m_{s}}{r_{s}}|_{s=s_i} = \min\limits_{\{m_{s^{'}}\}} \max \frac{F_{s_{'}}-m_{s^{'}}}{r_{s^{'}}}, \ \sum\limits_{s \in \mathcal{S}}m_s = M \right\}$
%		\EndProcedure
%	\end{algorithmic}
%\end{algorithm*}
%
%\begin{algorithm*}
%	\begin{algorithmic}[1]
		\Procedure{CACHE\_PLACEMENT}{}%{$\{ F^i, r_i ; \forall s_i \in \CS \}, \CK$}
		\State $\{m_i \} =  \arg\min\max\limits_{i} \frac{F-m_i F}{r_i} $
		
		\For{$s_i\in\mathcal{S}$} %\Comment{This is the beginning cache-arrangement.}
		
		\State $t_i = K \times m_i$ 
		
		\State $F^i \rightarrow \{f^{i}_{\CV_i} \; | \; \CV_i \subseteq \CK, |\CV_i| = t_i\}$
		
		\For{$k \in \CK$}
		\If{$k \in \CV$}
		    \State $\CZ_k \gets f^{i}_{\CV}$
		\EndIf
		\EndFor
		\EndFor
		\EndProcedure %\Comment{ This is the end of cache placement phase.}
	\end{algorithmic}
\end{algorithm}

\begin{algorithm}
    \caption{NCM-based Content Delivery}
	\begin{algorithmic}[1]
		\Procedure{DELIVERY}{}
		%{$\{F_{s_i},\dots,F_{s_j}\}$, \ $\{r_{s_i}, \ldots, r_{s_j}\}, \ \{\mathcal{Z}_1, \dots, \mathcal{Z}_K\}$}
		
		\State $t_c = \min\limits_{s_i \in \CS_u} t_i$
		\ForAll{$\CV_c \subseteq \CK, |\CV_c| = t_c+1$}
		    \State $X_c \gets 0$
		    \ForAll{$u_j \in \CV_c$}
		        \State $\alpha_j \gets \binom{t_j}{t_c}$
		        \State $Y_j \gets 0$
		        \State $\CV_{c \backslash j} = \CV_c \backslash \{u_j \}$
		        \ForAll{$\CV_j \subseteq \CK, |\CV_j| = t_j+1$}
		            \If{$\CV_{c \backslash j} \subseteq \CV_j$}
		                \State $f^{j,q}_{\CV_j} \gets$ \textsc{NewChunk}($f^{j}_{\CV_j}, \alpha_j$)
		                \State $Y_j \gets$ \textsc{Concatenate} $ (Y_j, f^{j,q}_{\CV_j})$ 
		            \EndIf
		        \EndFor
		        \State $X_c \gets$ \textsc{Nest} $(X_c, Y_j, r_j)$
		    \EndFor
		    \State Transmit $X_c$
		\EndFor
		
		%\State
		
		%\ForAll{$ s_i \in \CS_{u}$}
		%\ForAll{$ \CV \subseteq \CK, |\CV| = t_c$}
		%\State $\hat{f}^{s_i}_{\CV} = [NEW({f^{s_i}_{\CV_s}})]_{\{\forall \CV_s | \CV \subseteq \CV_s\}}$ 
		%\State \Comment{The function $NEW({f^{s}_{\mathcal{V}_s}})$ chooses a new part of $f^{s}_{\mathcal{V}_s}$ with size $\frac{|f^{s}_{\mathcal{V}_s}|}{\binom{t_s}{t_c}}$, and $[.]$ denotes concatenation.}
		%\EndFor
		%\EndFor
		
		%\ForAll{$\CD \subseteq \CK, |\CD|= t_c + 1$}

		%\State $X_{\CD} \gets *_{k \in \CD} f^{s_{u_k}}_{\CD \setminus k} $ 
		%\State \Comment{Nest each $f^{s_{u_k}}_{\CD \setminus k}$ together and transmit each file with the corresponding rate.}
		%\EndFor
		
		%\State \textbf{Transmit} $f^{s_{u_k}}_{\mathcal{D} \setminus k}$ with the rate $r_{s_{u_k}}$.
		\EndProcedure
		
	\end{algorithmic}
\end{algorithm}

\subsection{Content Delivery}
In the delivery phase, each user $u_j \in \CK$ is at a particular state $s_j \in \CS$. Based on the proposed cache placement, each state $s_j$ has specific $t_j$ and $r_j$ values. We set the common multicasting factor $t_c$ to be the minimum of $t_j$ values for all the users, i.e., $t_c = \min\limits_{u_j \in \CK}t_j$.

We deliver a nested codeword $X_{\CV_c}$ to any subset of users $\CV_c$ with size $t_c+1$ users. This nested codeword is designed such that the users with higher data rates (with smaller $t_j$ values) receive a larger data portion. Note that every user $u_j \in \CV_c$ has cached data parts $f^j_{\CV_j}$ for which $u_j \in \CV_j$, and needs to receive the rest of these data parts for a successful delivery. Let us denote the user set $\CV_c \backslash \{u_j\}$ with $\CV_{c \backslash j}$. During the transmission of $X_{\CV_c}$, we can deliver all data part(s) $f^j_{\CV_j}$ to $u_j$, for which $\CV_{c \backslash j} \subseteq \CV_j$. However, delivering all such data parts all together with $X_{\CV_c}$ causes $X_{\CV_c}$ to be \textit{inefficient}, i.e., there will be time instances during the transmission of $X_{\CV_c}$ in which some users in $\CV_c$ are not receiving any data. To solve this issue, we split every data part $f^j_{\CV_j}$ for which  $\CV_{c \backslash j} \subseteq \CV_j$ into smaller chunks, by splitting them into $\binom{t_j}{t_c}$ chunks denoted with $f^{j,q}_{\CV_j}$, where $q$ is an auxiliary index used to avoid transmitting the same data chunk multiple times. Finally, we concatenate all these data chunks.


In order to do so, for every user $u_j \in \CV_c$, we deliver a concatenation of smaller parts of its requested data available in the cache memory of other users in $\CV_c$, each with size $\binom{t_j}{t_c}$.


Next, for each state $s_j$, each file part $f^j_{\CV_j}$ is divided into $\binom{t_j}{t_c}$ smaller chunks.%, where $\mathcal{S}_u = \{s_{u_k}| \forall k \in \mathcal{K}\}$. 
Then, a sub-file $\hat{f}^{j}_{\CV}$ is created by concatenating a file chunk from each $\mathcal{V}_s$ such that $\mathcal{V} \subseteq \mathcal{V}_s$, where $\mathcal{V} \subseteq \mathcal{K}, |\mathcal{V}| = t_c$, i.e., $\hat{f}^{s}_{\mathcal{V}} = [NEW({f^{s}_{\mathcal{V}_s}})]_{\{\forall \mathcal{V}_s | \mathcal{V} \subseteq \mathcal{V}_s\}}$. Note that $|\mathcal{V}_s| \geq |\mathcal{V}|$, thus, there exist several $\mathcal{V} \subseteq \mathcal{V}_s$. Therefore, we use function $NEW(.)$ to make sure that unique file chunk is being dedicated to different subset $\mathcal{V}$ (see the example). Note that sub-file $\hat{f}^{s}_{\mathcal{V}}$ is available in the memory of all the users $k \in \mathcal{V}$.

For the delivery phase, $\binom{K}{t_c+1}$ transmission is required, where at each transmission $t_c+1$ users are being served with a common nested message. At each particular transmission, a nested message is transmitted to a subset of users, denoted as $\mathcal{D} \subseteq \mathcal{K}, |\mathcal{D}| = t_c+1$, as the following
\begin{equation}
    X_\mathcal{D} = *_{k \in \mathcal{D}} f^{s_{u_k}}_{\mathcal{D} \setminus k},
\end{equation}
where, $*$ is the nesting operation. Note that each user $k \in \mathcal{D}$ has all the sub-files $\{f^s_{\mathcal{V}}, \mathcal{V} \subset \mathcal{D}, |\mathcal{V}| = t_c\}$ but $f^{s_{u_k}}_{\mathcal{D} \setminus k}$, which must be transmitted with rate $r_{s_{u_k}}$. Thus, each user can cache out all the unwanted files in $X_\mathcal{D}$ with the help of its cache and decode its intended sub-file to recover the required file. Finally, the complete proposed cache placement and delivery scheme is summarised in algorithm~\ref{Alg_Main}.
\begin{theorem}
The proposed cache placement and delivery scheme satisfies all the users file requirement.
\begin{proof}
Consider user $k \in \mathcal{K}$ at state $s_{u_k}$, where it has $m_sF = \frac{t_{s_{u_k}} F}{K}$ [bits/Hz] available data in its cache and requires $f_{s_{u_k}} = F - m_{s_{u_k}}F = \frac{(K-t_{s_{u_k}})F}{K}$ remaining data from the transmitter. Based on the delivery scheme, each user receives $\binom{K-1}{t_c}$ sub-files $\{\hat{f}^{{s_{u_k}}}_{\mathcal{V}}, \mathcal{V} \subseteq \mathcal{K} \setminus k, |\mathcal{V}| = t_c$\} in the delivery phase. Each sub-file $\hat{f}^{{s_{u_k}}}_{\mathcal{V}}$ is the concatenated version of $\binom{K-t_c-1}{t_s-t_c}$ number of file-chunks with the size $\frac{F}{\binom{K}{t_s}\binom{t_{s_{u_k}}}{t_c}}$. As the result, $\frac{\binom{K-1}{t_c}\binom{K-t_c-1}{t_{s_{u_k}}-t_c}F}{\binom{K}{t_{s_{u_k}}}\binom{t_{s_{u_k}}}{t_c}}= \frac{(K-t_{s_{u_k}})F}{K}$ [bits/Hz] data is delivered through the transmitter and the remaining $\frac{t_{s_{u_k}}  F}{K}$ [bits/Hz] data is available in its cache.
\end{proof}
\end{theorem}
\subsection{Performance}
Though the placement and delivery scheme in this paper can be generalized, we use following assumptions for the performance analysis of the proposed method
\begin{itemize}
    \item The total available memory at each user is such that after solving~\eqref{cache-allocation} we have $m_s > 0, \forall s \in \mathcal{S}$.
    \item For each state $s \in \mathcal{S}$ we have integer $t_s = Km_s$, i.e., $t_s \in \{1,2, \dots, K\}$.
\end{itemize}
The generalized version of the cache placement and delivery scheme, along with the performance analysis is investigated in the simulation results (section~\ref{sec:simulation}).

\begin{lemma} \label{lemma:eqality}
At the optimal point the solution of~\eqref{cache-allocation} satisfies the following
\begin{equation} \label{eq:optimalms}
    \frac{F-m_sF}{r_s} = \frac{F-m_{s^{'}}F}{r_{s^{'}}}, \quad \forall \{s,s^{'}\} \in \mathcal{S}, s \neq s^{'}.
\end{equation}
    \begin{proof}
    The proof can be shown through contradiction. %Suppose at the optimally point there exist $s \in \mathcal{S}$ such that $\frac{F-m_s}{r_s} > \frac{F-m_{s^{'}}}{r_{s^{'}}}, \forall s^{'} \in \mathcal{S} \setminus s$, then by decreasing $m_s$ with $\delta$ and increasing the rest of states by $\frac{\delta}{|S|-1}$
    \end{proof}
\end{lemma}

\begin{lemma}\label{lemma:fs/rs}
At the optimal point the solution of~\eqref{cache-allocation} satisfies the following
\begin{equation} \label{eq: fs/rs}
    \frac{|f_s|}{r_s} = \frac{(S-M)F}{\sum\limits_{{s^{'}} \in \mathcal{S}}r_{s^{'}}}, \quad \forall s \in \mathcal{S}.
\end{equation}
where $|f_s| = F-m_sF$.
\begin{proof}
Since the total amount of available data for all the states is $SF$ and the total available cache dedicated to all the states at each user is $MF$, the sum of remaining data for all the states is
\begin{equation} \label{eq:sumfs}
    \sum\limits_{s \in \mathcal{S}}|f_s| = SF - MF.
\end{equation}
Now, using~\eqref{eq:optimalms} we have
\begin{equation} \label{eq:fsfsp}
    |f_s| = \frac{r_s}{r_{s^{'}}}|f_{s^{'}}|, \forall \{s, s^{'} \} \in \mathcal{S}.
\end{equation} 
Substituting~\eqref{eq:fsfsp} into~\eqref{eq:sumfs} and solving for $\frac{|f_{s^{'}}|}{r_{s^{'}}}$,~\eqref{eq: fs/rs} is achieved.
\end{proof}
\end{lemma}
Based on lemma~\ref{lemma:eqality} and lemma~\ref{lemma:fs/rs} the following statement holds.
\begin{theorem}\label{theorem:proposed transmission time}
the total delivery time of the proposed cache placement and delivery scheme is
\begin{equation}\label{eq:proposed transmission time}
    T_m = (\frac{K}{t_c + 1})\frac{(S-M)F}{\sum\limits_{s \in \mathcal{S}}r_s}.
\end{equation}
\begin{proof}
In general, each user $k \in \mathcal{K}$ at state $s_{u_k} \in \mathcal{S}$ requires $|f_{s_{u_k}}|$ [bits/Hz] to decode its intended data, which is delivered by $\binom{K-1}{t_c}$ transmissions (based on the proposed on the proposed delivery method). Since the transmitted data at each transmission has the same information, at each transmission $\frac{|f_{s_{u_k}}|}{\binom{K-1}{t_c}}$ [bits/Hz] with the rate $r_{s_{u_k}}$ [bits/Hz/s] is transmitted to user $k$. Thus, the total required time to serve user $k$ at each transmission is $\frac{1}{\binom{K-1}{t_c}}\frac{|f_{s_{u_k}}|}{r_{s_{u_k}}}$. Now, using~\eqref{eq: fs/rs} it can be deduced that each transmission takes exactly $\frac{1}{\binom{K-1}{t_c}}\frac{(S-M)F}{\sum\limits_{s \in \mathcal{S}}r_s}$ seconds. Using the fact that the total number of required transmissions to serve all the users is $\binom{K}{t_c + 1}$ and each transmission takes $\frac{1}{\binom{K-1}{t_c}}\frac{(S-M)F}{\sum\limits_{s \in \mathcal{S}}r_s}$ seconds, theorem~\ref{theorem:proposed transmission time} is proved.
\end{proof}
\end{theorem}
\begin{lemma}
The delivery time of the proposed delivery scheme satisfies the following statement
\begin{equation} \label{eq:tm/tu}
    \frac{T_m}{T_u} = \frac{1}{t_c+1}, \quad \forall s \in \mathcal{S}_u,
\end{equation}
where $T_u$ is the delivery time of unicasting.
\begin{proof}
In unicasting, only one user is served at each transmission. Thus, the total delivery time is $T_u = \sum\limits_{s \in \mathcal{S}_u}\frac{f_s}{r_s}$. Using~\eqref{eq: fs/rs}, the unicasting delivery time is $T_u = K\frac{(S-M)F}{\sum\limits_{s \in \mathcal{S}}r_s}$.
\end{proof}
\end{lemma}

\begin{corollary}
When users are in locations with low transmission rates, they can benefit from cache with higher $m_s$. As a result, $t_c$ will be larger, which will increase the proposed delivery gain and compensates for the low transmission rates.
\end{corollary}
\begin{theorem}
The proposed cache placement and delivery scheme has a bounded average delivery time gap from any optimal cache placement and delivery scheme. 
\begin{proof}
See arxiv.
\end{proof}
\end{theorem}


==> Uneven Cache Placement - ISIT _extend/NewScheme_remaster.tex <==
Similar to other centralized coded caching schemes, our new location-dependent scheme also works in two distinct phases, 1) cache placement and 2) content delivery. %For better clarification, throughout the discussions we frequently refer to the example network considered in Section~\ref{section:example_net}.
%\textbf{Its better to state our assumption for $t$ and $m$ here.}

\subsection{Cache Placement}
During the placement phase, the users' cache memories are filled up with useful data to minimize the duration of the content delivery phase. However, the content placement phase is carried out without any prior knowledge of users' spatial distribution in the delivery phase. As defined in Section~\ref{section:system_model}, we assume the application environment is split into $S$ states, and a location-dependent multimedia file of size one normalized data unit is required to reconstruct the static FoV of each state.

%Let us use $W(j)$ to denote the file required for reconstructing the FoV of the state $j \in \CS$. 
Before proceeding with the data placement, we first use a \textit{memory allocation} process to determine the dedicated amount of cache memory for storing (parts of) $W(j)$ at each user. Since there is no prior knowledge about the users' spatial realizations in the delivery phase, we minimize the maximum delivery time for a single user assuming uniform access probability for all the states. Let us use $m(j)$ to denote the normalized cache size at each user allocated to storing (parts of) $W(j)$. Since the size of $W(j)$ is normalized to one data unit, a user in state $j$ needs to receive $1-m(j)$ data units over the wireless link to reconstruct the FoV of state $j$. As a result, data delivery to state $j$ needs $T(j) = \frac{1-m(j)}{r(j)}$ seconds. Hence, the memory allocation for minimizing the maximum delivery time is found by solving the following linear program (LP):\footnote{Note that the achievable delivery time $\gamma$ can be controlled through $F$ and $B$ to meet the application's real-time requirements. In this regard, the solution of~\eqref{cache-allocation} can determine the maximum achievable QoE of different states (i.e., the maximum value of $F$ such that the constraints are met), using bisection over $F$ (and/or $B$). }
\begin{equation}
\begin{aligned}
\label{cache-allocation}
 \text{LP} \ : \quad &\min_{m(j), \gamma \ge 0}  \gamma\\
&\textrm{s.t.} \quad  \frac{1-m(j)}{r(j)} \leq \gamma, \ \forall j \in \CS, \\
& \sum_{j \in \CS} m(j) = M.
\end{aligned}
\end{equation}
%
%\textbf{Add here discussion how this can be used to maximize the QoE given the delivery time constraints! Can be done offline using bisection over F (and/or B).}


After the memory allocation process, we store data in the cache memories of the users following the same method proposed in~\cite{maddah2014fundamental}. In this regard, for every $j\in\CS$ we split $W(j)$ into~$\binom{K}{t(j)}$ sub-files denoted by $W_{\CV(j)}(j)$, where $t(j) = K m(j)$ and $\CV(j)$ can be any subset of the user set $\CK$ with $|\CV(j)| = t(j)$.\footnote{Here we assume for every $j\in\CS$, $m(j)>0$ and $t(j)$ is an integer. In the next sections, it is briefly discussed what happens if these constraints are not met. However, a detailed discussion is left for the extended version.} Then, at the cache memory of user $i \in \CK$, we store $W_{\CV(j)}(j)$ for every state $j \in \CS$ and set $\CV(j) \ni i$. The cache placement procedure is outlined in Algorithm~\ref{Alg:placement}. 

\begin{exmp}
\label{exmp:placement}
Consider an application with $K=4$ users, where the environment is split into $S=5$ states and for each state, the required data size is $F=400$ Megabytes. Each user has a cache size of $900$ Megabytes, and hence, the normalized cache size is $M = 2.25$ data units. The spatial distribution of the achievable rate (assuming $B=F$) and its resulting memory allocation are as shown in Figure~\ref{fig:rate&cache_distribution}. It can be easily verified that $t(1) = t(5) = 1$, $t(2) = t(4) = 2$, and $t(3)=3$. As a result, $W(1)$, $W(3)$ and $W(5)$ should be split into four sub-files, while $W(2)$ and $W(4)$ are split into six sub-files. The resulting cache placement is visualized in Figure~\ref{fig:cache pool}.
%\begin{figure}[t]
%    \centering 
%    \includegraphics[width=1\columnwidth,keepaspectratio]{Figs/sample pic.pdf}
%    \caption{Location-specific rate distribution and corresponding cache allocation.}
%\label{fig:rate&cache_distribution}
%\end{figure}
\begin{figure}[t]
\input{Figures/Fig2}
\end{figure}
\input{PlacementFigure}

%\begin{figure}[t]
%    \centering 
%    \includegraphics[width=1\columnwidth,keepaspectratio]{Figs/location_specific_cacheplacement.pdf}
%    \caption{Location-specific cache pool arrangement.}
%\label{fig:cache pool}
%\end{figure}
\end{exmp}

As $W(j)$ is split into $\binom{K}{t(j)}$ sub-files and $\binom{K-1}{t(j)-1}$ sub-files are stored in the cache memory of each user, the total memory size dedicated to $W(j)$ at each user is
\begin{equation}
    \frac{\binom{K-1}{t(j)-1}}{\binom{K}{t(j)}} = \frac{t(j)}{K} = m(j) \; ,
\end{equation} 
and hence, the proposed algorithm satisfies the cache size constraints.
Note that, in comparison with~\cite{maddah2014fundamental}, here the required files in each state are considered as a separate library, and the cache placement algorithm in~\cite{maddah2014fundamental} is performed for each state independent of the others. Also, different from the existing works, here, files of different locations have distinct $t(j)$ values, which should be carefully considered in the delivery phase. For notational simplicity, throughout the paper we ignore the brackets and separators while explicitly writing $\CV(j)$, i.e., $W_{i \, k}(j) \equiv W_{\{i,k\}}(j)$. 





\begin{algorithm}[t]
\small
	\caption{Location-based cache placement}
	\begin{algorithmic}[1]
		\Procedure{CACHE\_PLACEMENT}{}%{$\{ F^i, r_i ; \forall s_i \in \CS \}, \CK$}
		\State $\{m(j) \} =$ The result of the LP problem in~\eqref{cache-allocation}% \arg\min\max\limits_{i} \frac{F-m_i F}{r_i} $
		
		\ForAll{$j \in \CS$} %\Comment{This is the beginning cache-arrangement.}
		
		\State $t(j) = K \times m(j)$ 
		
		\State $W(j) \rightarrow \{W_{\CV(j)}(j) \; | \; \CV(j) \subseteq \CK, |\CV(j)| = t(j)\}$
		
		\ForAll{$\CV(j)$}
		\ForAll{$i \in \CK$}
		\If{$i \in \CV(j)$}
		    \State Put $W_{\CV(j)}(j)$ in the cache of user $i$
		\EndIf
		\EndFor
		\EndFor
		\EndFor
		\EndProcedure 
	\end{algorithmic}
	\label{Alg:placement}
\end{algorithm}

%------------------------------------------------------
\subsection{Content Delivery}
At the beginning of the delivery phase, every user $i \in \CK$ reveals its requested file $W_i \equiv W(s_i).$\footnote{Note that we have used $W(j)$ to represent the file required for reconstructing the FoV of the state $j$, and $W_i$ to denote the file requested by user~$i$. The same convention is used for all notations in the text.} Note that $W_i$ depends on the state $s_i$ where user $i$ is located. The server then builds and transmits several \textit{nested} codewords, such that after receiving the codewords, all users can reconstruct their requested files. From the system model, user $i$ requires a total amount of one normalized data unit to reconstruct $W_i$. However, a subset of this data, with size $m_i \equiv m(s_i)$ data units, is available in the cache of user $i$. Since each user might be in a different state with distinct $t(j)$, the conventional delivery scheme of~\cite{maddah2014fundamental} is no longer applicable, and a new delivery mechanism is required to achieve a proper multicasting gain.

\begin{algorithm}[t]
\small
    \caption{NCM-based Content Delivery}
	\begin{algorithmic}[1]
		\Procedure{DELIVERY}{}
		
		\State $\hat{t} = \min_{i \in \CK} t_i$
		\ForAll{$\CU \subseteq \CK : |\CU| = \hat{t}+1$}
		    \State $X_{\CU} \gets 0$
		    \ForAll{$i \in \CU$}
		        \State $\alpha_i \gets \binom{t_i}{\hat{t}}$, $Y_{\CU,i} \gets 0$, $\CU_{-i} \gets \CU \backslash \{i \}$
		        \ForAll{$\CV_i \subseteq \CK : |\CV_i| = t_i+1$}
		            \If{$\CU_{-i} \subseteq \CV_i$, $i \not\in \CV_i$}
		                \State $W_{\CV_i,i}^q \gets$ \textsc{Chunk}($W_{\CV_i,i}, \alpha_i$)
		                \State $Y_{\CU,i} \gets$ \textsc{Concat} $ (Y_{\CU,i}, W_{\CV_i,i}^q)$ 
		            \EndIf
		        \EndFor
		        \State $X_{\CU} \gets$ \textsc{Nest} $(X_{\CU}, Y_{\CU,i}, r_i)$
		    \EndFor
		    \State Transmit $X_{\CU}$
		\EndFor
		\EndProcedure
	\end{algorithmic}
	\label{Alg:Delivery}
\end{algorithm}

The new delivery algorithm for the proposed setup is outlined in Algorithm~\ref{Alg:Delivery}. During the delivery phase, the server transmits a nested codeword $X_{\CU}$ for every subset of users $\CU$ with $|\CU|= \hat{t} +1$, where $\hat{t}$ is the \textit{common cache ratio} defined as $\hat{t} = \min_{i \in \CK} t_i$, and $t_i \equiv t(s_i)$. From the placement phase, we recall that the file $W_i$ intended for user $i \in \CU$ is split into sub-files $W_{\CV(s_i),i}$.
%, where $\CV(s_i) := \{ \CV \ | \ \CV \subseteq \CK$, $|\CV(s_i)| = t_i\}$. 
Let us define $\CU_{-i} \equiv \CU \setminus \{i\}$ and consider a user $k \in \CU_{-i}$. All the sub-files $W_{\CV(s_i),i}$ for which $k \in \CV(s_i)$ are already available in the cache memory of user $k$. Thus, by transmitting (part of) every sub-file $W_{\CV(s_i),i}$ for which $\CU_{-i} \subseteq \CV(s_i)$ and $i \not\in \CV(s_i)$, a portion of $W_i$ is delivered to user $i$ without causing any interference at other users $k \in \CU_{-i}$.

\begin{exmp}
\label{exmp:interference-free-delivery}
Consider the network in Example~\ref{exmp:placement}, for which the cache placement is visualized in Figure~\ref{fig:cache pool}. Assume in a specific time slot, $s_1 = 1$, $s_2 =2$, $s_3 =4$, $s_4 = 5$. Denoting the set of requested sub-files for user $i$ with $\CT_i$ and assuming $A \equiv W(1)$, $B \equiv W(2)$, $C \equiv W(4)$, $D \equiv W(5)$, we have
\begin{equation}
    \begin{aligned}
    \CT_1 &= \{ A_{2}, A_{3}, A_{4} \}, \qquad
    \CT_2 = \{ B_{13}, B_{14}, B_{34} \}, \\
    \CT_3 &= \{ C_{12}, C_{14}, C_{24} \}, \quad
    \CT_4 = \{ D_{1}, D_{2}, D_{3} \}. \\
    \end{aligned}
\end{equation}
Note that, the size of the sub-files of $A,B,C,D$ are $\frac{1}{4}, \frac{1}{6}, \frac{1}{6}, \frac{1}{4}$ data units, respectively. The common cache ratio is $\hat{t} = 1$, and hence, during each transmission we deliver data to $\hat{t}+1 = 2$ users.
%, and we need $\binom{4}{2} = 6$ transmissions in total. 
Let us consider the case $\CU = \{1,2\}$. The codeword $X_{12}$ is supposed to deliver a portion of the requested data to users $1$ and $2$ interference-free. This is done by including (parts of) $A_{2}$, $B_{13}$, $B_{14}$ in $X_{12}$. As can be seen from Figure~\ref{fig:cache pool}, user $1$ has $B_{13}$ and $B_{14}$ in its cache memory, and so it can remove them from its received data and decode (part of) $A_{2} \in \CT_1$ interference-free. Similarly, user $2$ can remove $A_{2}$ using its cache contents and decode (parts of) $B_{13},B_{14} \in \CT_2$ interference-free. The coding procedure is explained in more details in Example~\ref{exmp:coding-procedure}.
\end{exmp}

As illustrated in Example~\ref{exmp:interference-free-delivery}, 
due to the proposed location-dependent cache placement, the value of $t_i$ (and hence, the length of the transmitted sub-files) might be different for various users. Moreover, we may find more than one sub-file to be transmitted to user $i \in \CU$. We address these issues by introducing a normalizing factor $\alpha_i = \binom{t_i}{\hat{t}}$ and two auxiliary functions $\textsc{Chunk}$ and $\textsc{Concat}$. Whenever $t_i > \hat{t}$ for user $i \in \CU$, we first split every sub-file intended for user $i$ into $\alpha_i$ smaller \textit{chunks} (denoted by $W_{\CV(s_i),i}^q$ in Algorithm~\ref{Alg:Delivery}). Then, we \textit{concatenate} a selection of these chunks to create the part of $X_{\CU}$ intended for user $i$, represented by $Y_{\CU,i}$. The function $\textsc{Chunk}$ ensures none of the chunks of a sub-file is sent twice, and the function $\textsc{Concat}$ creates a bit-wise concatenation of the given chunks. The final codeword $X_{\CU}$ is created by nesting $Y_{\CU,i}$ for every user $i \in \CU$. This is shown by the auxiliary function $\textsc{Nest}$ in Algorithm~\ref{Alg:Delivery}. Note that due to the nesting, every $Y_{\CU,i}$ can be transmitted with rate $r_i \equiv r(s_i)$ (c.f.~\cite{tang2011full}). 

\begin{exmp}
\label{exmp:coding-procedure}
Following Example~\ref{exmp:interference-free-delivery}, let us review how the codeword $X_{12}$ is built. This codeword includes (parts of) $A_{2}$, $B_{13}$, $B_{14}$, intended for users $1$ and $2$. However, the size of $A_2$ is $\frac{1}{4}$, while $B_{13},B_{14}$ are both $\frac{1}{6}$ data units. To solve this issue, we use normalizing factors $\alpha_1 = 1$ and $\alpha_2 = 2$, and build
\begin{equation}
    X_{12} = A_2 * \textsc{Concat} (B_{13}^{1}, B_{14}^{1}) \; ,
\end{equation}
where the operator ($*$) denotes the nesting operation and superscripts are used to differentiate various chunks of a sub-file. The nesting operation in $X_{12}$ is performed such that $A_2$ and $\textsc{Concat} (B_{13}^{1}, B_{14}^{1})$ are delivered with rates $r_1 = 3$ and $r_2 = 2$ data units per second, respectively. As a result, this codeword is delivered in $\max(\frac{1}{3} \times \frac{1}{4}, \frac{1}{2} \times \frac{2}{12}) = \frac{1}{12}$ seconds. 
Similarly, as $\alpha_3 = 2$ and $\alpha_4 = 1$, we have
\begin{equation}
    \begin{aligned}
    X_{13} &= A_3 * \textsc{Concat}(C_{12}^{1},C_{14}^{1}) \; , \qquad X_{14} = A_4 * D_1 \; , \\
    X_{23} &= \textsc{Concat}(B_{13}^{2} \; B_{34}^{1}) * \textsc{Concat}(C_{12}^{2} \; C_{24}^{1}) \; , \\
    X_{24} &= \textsc{Concat}(B_{14}^{2} \; B_{34}^{2}) * D_2 \; , \\
    X_{34} &= \textsc{Concat}(C_{14}^{4} \; C_{24}^{4}) * D_3 \; , \\
    \end{aligned}
\end{equation}
where each transmission requires $\frac{1}{12}$ seconds. Thus, the total delivery time is $\frac{6}{12}$ seconds. In comparison, it can be seen that the delivery time would be doubled without multicasting.
\end{exmp}

%Next, for each state $s_j$, each file part $f^j_{\CV_j}$ is divided into $\binom{t_j}{t_c}$ smaller chunks.%, where $\mathcal{S}_u = \{s_{u_k}| \forall k \in \mathcal{K}\}$. 
%Then, a sub-file $\hat{f}^{j}_{\CV}$ is created by concatenating a file chunk from each $\mathcal{V}_s$ such that $\mathcal{V} \subseteq \mathcal{V}_s$, where $\mathcal{V} \subseteq \mathcal{K}, |\mathcal{V}| = t_c$, i.e., $\hat{f}^{s}_{\mathcal{V}} = [NEW({f^{s}_{\mathcal{V}_s}})]_{\{\forall \mathcal{V}_s | \mathcal{V} \subseteq \mathcal{V}_s\}}$. Note that $|\mathcal{V}_s| \geq |\mathcal{V}|$, thus, there exist several $\mathcal{V} \subseteq \mathcal{V}_s$. Therefore, we use function $NEW(.)$ to make sure that unique file chunk is being dedicated to different subset $\mathcal{V}$ (see the example). Note that sub-file $\hat{f}^{s}_{\mathcal{V}}$ is available in the memory of all the users $k \in \mathcal{V}$.

%For the delivery phase, $\binom{K}{t_c+1}$ transmission is required, where at each transmission $t_c+1$ users are being served with a common nested message. At each particular transmission, a nested message is transmitted to a subset of users, denoted as $\mathcal{D} \subseteq \mathcal{K}, |\mathcal{D}| = t_c+1$, as the following
%\begin{equation}
%    X_\mathcal{D} = *_{k \in \mathcal{D}} f^{s_{u_k}}_{\mathcal{D} \setminus k},
%\end{equation}
%where, $*$ is the nesting operation. Note that each user $k \in \mathcal{D}$ has all the sub-files $\{f^s_{\mathcal{V}}, \mathcal{V} \subset \mathcal{D}, |\mathcal{V}| = t_c\}$ but $f^{s_{u_k}}_{\mathcal{D} \setminus k}$, which must be transmitted with rate $r_{s_{u_k}}$. Thus, each user can cache out all the unwanted files in $X_\mathcal{D}$ with the help of its cache and decode its intended sub-file to recover the required file. Finally, the complete proposed cache placement and delivery scheme is summarised in algorithm~\ref{Alg:placement}.
\begin{thm}
Using the proposed cache placement and content delivery algorithms, every user receives its requested data.
\end{thm}
\begin{proof}
A user $i \in \CK$ needs a total amount of one (normalized) data unit to reconstruct its requested file $W_i$. If the user is in state $s_i$, $m(s_i)$ data units are available in its cache memory, and hence it needs to receive $1-m(s_i) = 1 - \frac{t_i}{K}$ data units from the server. As detailed in the delivery algorithm, user $i$ receives parts of its requested data in $\binom{K-1}{\hat{t}}$ transmissions. Consider one such transmission, where the codeword $X_{\CU}$ is transmitted to the users in $\CU \ni i$. During this transmission, user $i$ receives $Y_{\CU,i}$, which is built through concatenation of $\binom{K-\hat{t}-1}{t_i - \hat{t}}$ chunks, each with size
%\begin{equation}
    $\nicefrac{1}{\alpha_i \binom{K}{t_i}} = \nicefrac{1}{\binom{K}{t_i} \binom{t_i}{\hat{t}}}$
%\end{equation}
data units. As a result, the total data size delivered to user $i$ from the server is
\begin{equation}
    \frac{ \binom{K-1}{\hat{t}} \binom{K-\hat{t}-1}{t_i - \hat{t}} }{ \binom{K}{t_i} \binom{t_i}{\hat{t}} } = \frac{K-t_i}{K} = 1 - \frac{t_i}{K} \; ,
\end{equation}
and the proof is complete.
\end{proof}

\section{Performance Analysis}
\label{section:performance}
We discuss the performance of the proposed scheme assuming that for every state $j \in \CS$, $t(j)$ is a positive integer. Then we briefly review what happens if this assumption is relaxed.


\begin{figure*}[ht]
\begin{minipage}{0.32\linewidth}
%\centering  % redundant
\input{Figures/Fig4}
%\caption{caption1}
\label{fig:figure1}
\end{minipage}%
\hfill% not: "\hspace{0.5cm}"
\begin{minipage}{0.3\linewidth}
%\centering  % redundant
\input{Figures/Fig5}
%\caption{caption2}
\label{fig:figure2}
\end{minipage}%
\hfill% not: "\hspace{0.5cm}"
\begin{minipage}{0.3\linewidth}
%\centering  % redundant
\input{Figures/Fig6}
%\caption{caption3}
\label{fig:figure3}
\end{minipage}
\vspace{-15pt}
\end{figure*}


\begin{lem} \label{lemma:eqality}
For every two states $j,j' \in \CS$, the result of the memory allocation problem in~\eqref{cache-allocation} satisfies
\begin{equation} \label{eq:optimalms}
    \frac{1-m(j)}{r(j)} = \frac{1-m(j')}{r(j')}\;, \quad  \frac{1-m(j)}{r(j)} = \frac{S-M}{\sum_{j' \in \CS} r(j')} \; .
\end{equation}
\end{lem}
\begin{proof}
The first equality can be simply proved by contradiction.
%Proving the first equality is straightforward and can be achieved through contradiction. % Using simple operations, it results in $1-m(j') = \frac{1-m(j)}{r(j)} r(j')$. However, we know $\sum_{j\in\CS} m(j) = M$, and hence, $\sum_{j\in\CS}1-m(j) = S-M$. Substituting this into the former equality we can simply write
Using this equality, for the second one we can write
\begin{equation}
    \frac{1-m(j)}{r(j)} \sum_{j'\in\CS} r(j') = \sum_{j'\in\CS} 1-m(j') = S-M  \; ,
\end{equation}
and the proof is complete.
\vspace{-5pt}
%For the other one, we first use the first equality to write $1-m(j') = \frac{1-m(j)}{r(j)} r(j')$. However, we know $\sum_{j\in\CS} m(j) = M$, and hence, $\sum_{j\in\CS}1-m(j) = S-M$. Substituting this 
%For the other one, since $\sum_{j\in\CS} m(j) = M$ we have $\sum_{j\in\CS}1-m(j) = S-M$. However, using the first equality we can write
%\begin{equation} \label{eq:fsfsp}
%    $1-m(j') = \frac{1-m(j)}{r(j)} r(j'), \quad \forall j,j' \in \CS \;$ ,
%\end{equation}
%and hence
%for every $j\in\CS$, and the proof is complete.
\end{proof}

\begin{thm}\label{theorem:proposed transmission time}
Total delivery time of the proposed scheme, denoted by $T_m$, is calculated as
\begin{equation}\label{eq:proposed transmission time}
    T_m = \frac{K}{\hat{t} + 1} \frac{S-M}{\sum_{j \in \CS}r(j)} \; .
\end{equation}
\end{thm}
\begin{proof}
A user $i \in \CK$ receives $1-m(s_i)$ data units from the server through $n = \binom{K-1}{\hat{t}}$ transmissions. However, as the same procedure is followed to build $Y_{\CU,i}$ for every $\CU \ni i$, the data size delivered to user $i$ is the same for all these transmissions. Moreover, this user is always served with the rate $r_i$, and hence, it needs $T_i = \frac{1}{n} \frac{1-m(s_i)}{r(i)}$ seconds to receive every data part. Using Lemma~\ref{lemma:eqality}, we can rewrite $T_i$ as 
%\begin{equation}
%\label{eq:transmission_time_global}
    $T_i = \frac{1}{n} \frac{S-M}{\sum_{j \in \CS} r(j)}$,
%\end{equation}
which means the time required for all the transmissions is the same and independent of the user selection. As in the delivery phase there exist a total number of $\binom{K}{\hat{t}+1}$ transmissions, the total delivery time is
\begin{equation}
    T_m = \frac{\binom{K}{\hat{t}+1}}{\binom{K-1}{\hat{t}}} \frac{S-M}{\sum_{j \in \CS}r(j)} = \frac{K}{\hat{t} + 1}\frac{S-M}{\sum_{j \in \CS}r(j)} \; ,
\end{equation}
and the proof is complete.
\end{proof}

\begin{thm}
\label{thm:time_gain}
Compared with unicasting, the proposed scheme enables a reduction in the delivery time by a factor of $\hat{t}+1$.
\end{thm}
\begin{proof}
In case of unicasting, a user $i$ gets $1-m(s_i)$ data units with the rate $r_i$, and hence, the total delivery time is equal to
%\begin{equation}
    $T_u = \sum_{i \in \CK} \frac{1-m(s_i)}{r_i}$.
%\end{equation}
However, using Lemma~\ref{lemma:eqality} we have
\begin{equation}
    T_u = \sum_{i \in \CK} \frac{S-M}{\sum_{j\in\CS}r(j)} = K\frac{S-M}{\sum_{j\in\CS}r(j)} \; ,
\end{equation}
which is $\hat{t}+1$ times larger than the $T_m$ value in~\eqref{eq:proposed transmission time}.% as calculated in Theorem~\ref{theorem:proposed transmission time}.
%Comparing $T_u$ with the delivery time of the proposed scheme (calculated in Theorem~\ref{theorem:proposed transmission time}), the proof is complete.
\end{proof}

\begin{cor} 
The proposed scheme becomes more efficient if $\hat{t}$ is larger.
%As $\hat{t}$ becomes larger, the proposed scheme becomes more efficient. 
This happens, for example, when more users are located in states with poor channel conditions.% or when all users are in proximity to each other.
%When more users are located in states with poor channel conditions, $\hat{t}$ is larger, and hence, the proposed method provides higher transmission efficiency. In other words, our method performs better as we are more limited by the rate. 
%When users are in a proximity to each other and with relatively poor channel conditions.... ...., the value of $\hat{t}$ increases and the coded caching gain would be larger.
\end{cor}

\begin{thm}
Under the assumption of uncoded cache placement, the proposed delivery time in~\eqref{eq:proposed transmission time} is within a bounded gap from any optimal scheme and satisfies
\begin{equation} \label{bound:performance_gap_mn}
    \frac{T_m}{T^{*}} \le \frac{\bar{r}}{(\hat{m}+\frac{1}{K}) \sum_{j \in \CS}r(j)}\left(\frac{S}{K}+M\right) \; ,
\end{equation}
where $\bar{r} = \max_{j \in \CS} r(j)$, $\hat{m} = \min_{j \in \CS} m(j)$, and $T^*$ is the optimal delivery time with uncoded cache placement. 
\end{thm}

\begin{proof}
For proof, we use optimality results provided for the original scheme of~\cite{maddah2014fundamental}. Note that if $r(j)$ is the same for every state $j \in \CS$, our scheme becomes equivalent to~\cite{maddah2014fundamental}, with library size $S$ and coded caching gain $\frac{KM}{S}$. Moreover, in~\cite{yu2017exact}, it is shown that under the assumption of uncoded cache placement, the original coded caching scheme in~\cite{maddah2014fundamental} is exactly optimal. So, we can provide an upper bound for the optimal delivery time in our setup by simply assuming that the achievable rate at every state is the same and equal to $\bar{r}$. Using the delivery time expressions in~\cite{maddah2014fundamental}, we can write
\begin{equation}
    \frac{K(S-M)}{S+KM} \frac{1}{\bar{r}} \le T^* \; ,
\end{equation}
which, together with~\eqref{eq:proposed transmission time}, results in
\begin{equation}
\label{eq:bound_int_relation}
    \frac{T_m}{T^*} \le \frac{K(S-M)}{(\hat{t}+1)\sum_{j \in \CS} r(j)} \frac{S+KM}{K(S-M)} \bar{r} \; .
\end{equation}
However, as we have
\begin{equation}
    \hat{t} = \min_{i \in \CK} t(s_i) \ge \min_{j \in \CS} t(j) = K \min_{j \in \CS} m(j) = K \hat{m} \; ,
\end{equation}
we can simply substitute $\hat{t}$ with $K \hat{m}$ in~\eqref{eq:bound_int_relation}, to reach the upper bound proposed in~\eqref{bound:performance_gap_mn}. Note that the right hand side expression in~\eqref{bound:performance_gap_mn} approaches to
\begin{equation}
    \frac{\bar{r}M}{\hat{m}\sum_{j \in \CS} r(j)}
\end{equation}
as $K \rightarrow \infty$, and is bounded by 
\begin{equation}
    \frac{\bar{r}}{K(\hat{m}+\frac{1}{K})\min_{j\in\CS}r(j)}
\end{equation}
as $S \rightarrow \infty$. Hence, in both cases, the proposed delivery time in our scheme is within a bounded gap from any optimal scheme, and the proof is complete.



%To prove~\eqref{bound:performance_gap_mn} we first show that the achievable delivery time of the~\cite{maddah2014fundamental} for the proposed setting is lower bounded by
%\begin{equation}
%    T_x \geq \frac{K(S-M)}{S-KM}\frac{1}{\max_{i \in \mathcal{S}}r(i)},
%\end{equation}
%where we have assumed that the achievable rate for all the states is the same and equal to $\max_{i \in \mathcal{S}}r(i)$. Now, using~\eqref{eq:proposed transmission time} we can state
%\begin{equation}
%    \frac{T_m}{T_x} \leq \frac{\max_{i \in \mathcal{S}}r(i)}{(1 + K\min_{s \in \mathcal{S}}m(s))\sum_{j \in \CS}r(j)}\left(K\left(\frac{S}{K}-M\right)\right),
%\end{equation}
%or equivalently we can write the following
%\begin{equation}
%    T_m \leq \frac{\max_{i \in \mathcal{S}}r(i)}{(\min_{s \in \mathcal{S}}m(s))\sum_{j \in \CS}r(j)}\left(\frac{S}{K}-M\right)T_x.
%\end{equation}
%Now, following the fact that $T_X \leq \frac{X_{mn}}{\max_{i \in \mathcal{S}}r(i)}$ ($X_{mn} = \frac{K(1-\frac{M}{S})}{1+\frac{KM}{S}}$), and $T^{*} \geq \frac{\overline{X}}{\max_{i \in \mathcal{S}}r(i)}$, we can write the following
%\begin{equation}
%    \frac{T_m}{T^{*}} \leq \frac{\max_{i \in \mathcal{S}}r(i)}{\min_{j \in \mathcal{S}}m(j)}\left(\frac{S}{K}-M\right) \frac{X_{mn}}{\overline{X}}.
%\end{equation}
%Using the fact that for uncoded placement and delivery schemes the fraction $\frac{X_{mn}}{\overline{X}}$ is proved to be 1, the claim is proved.
\end{proof}
%\begin{cor}
%The gap~\eqref{bound:performance_gap_mn} does not increase unboundedly with the number of users, i.e., $\lim_{K \rightarrow \infty}\frac{T_m}{T^{*}} \leq \frac{\overline{r}M}{\hat{m}\sum_{j \in \mathcal{S}}r(j)}$. Moreover, the gap does not increase unboundedly with the number of states, i.e., $\lim_{S \rightarrow \infty}\frac{T_m}{T^{*}} \leq \frac{\overline{r}}{K(\hat{m}+\frac{1}{K})\underline{r}}$, where $\underline{r} = \min_{j \in \mathcal{S}}r(j)$. 
%\end{cor}


It can be shown that, if all $t(j)$ values are not integers, all the results provided in this section still hold. However, if $m(j)=0$ for some $j \in \CS$, the reduction factor in delivery time, proposed in Theorem~\ref{thm:time_gain}, is no longer valid. This is because, in such a case, it is not always possible to deliver all the required data through multicasting (some missing parts should be delivered by unicasting). %Still, it can be shown that the performance gap of the proposed scheme with the optimal solution would be bounded. %Due to the lack of space, a detailed discussion on these results is left for the extended version of this paper.


==> Uneven Cache Placement - ISIT _extend/PlacementFigure.tex <==
\begin{figure}
    \smaller
    \centering
    \resizebox{0.7\columnwidth}{!}{%
    \begin{tabular}{c}
        \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
            \cline{2-13}
            \multicolumn{1}{c|}{} & \multicolumn{3}{c|}{\tiny$\,\qquad W_1(j) \qquad$} & \multicolumn{3}{c|}{\tiny$\,\qquad W_2(j) \qquad$} & \multicolumn{3}{c|}{\tiny$\,\qquad W_3(j) \qquad$} & \multicolumn{3}{c|}{\tiny$\,\qquad W_4(j) \qquad$} \\
            \hline
            \multirow{4}{*}{\rotatebox[origin=c]{90}{\small $j=1,5$}} & \multicolumn{3}{c|}{\cellcolor{gray!50}} & 
            \multicolumn{3}{c|}{} & 
            \multicolumn{3}{c|}{} & 
            \multicolumn{3}{c|}{} & user $1$ \\
            \cline{2-14}
            & \multicolumn{3}{c|}{} & 
            \multicolumn{3}{c|}{\cellcolor{gray!50}} & 
            \multicolumn{3}{c|}{} & 
            \multicolumn{3}{c|}{} & user $2$ \\
            \cline{2-14}
            & \multicolumn{3}{c|}{} & 
            \multicolumn{3}{c|}{} & 
            \multicolumn{3}{c|}{\cellcolor{gray!50}} & 
            \multicolumn{3}{c|}{} & user $3$ \\
            \cline{2-14}
            & \multicolumn{3}{c|}{} & 
            \multicolumn{3}{c|}{} & 
            \multicolumn{3}{c|}{} & 
            \multicolumn{3}{c|}{\cellcolor{gray!50}} & user $4$ \\
            \hline
            \multicolumn{14}{c}{}\\[-0.7em]
        \end{tabular} \\
        \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
            \cline{2-13}
            \multicolumn{1}{c|}{} & \multicolumn{2}{c|}{\tiny$W_{12}(j)$} & \multicolumn{2}{c|}{\tiny$W_{13}(j)$} & \multicolumn{2}{c|}{\tiny$W_{14}(j)$} & \multicolumn{2}{c|}{\tiny$W_{23}(j)$} & \multicolumn{2}{c|}{\tiny$W_{24}(j)$} & \multicolumn{2}{c|}{\tiny$W_{34}(j)$}  \\
            \hline
            \multirow{4}{*}{\rotatebox[origin=c]{90}{\small $j=2,4$}} & \multicolumn{2}{c|}{\cellcolor{gray!50}} & 
            \multicolumn{2}{c|}{\cellcolor{gray!50}} & 
            \multicolumn{2}{c|}{\cellcolor{gray!50}} & 
            \multicolumn{2}{c|}{} & \multicolumn{2}{c|}{} & \multicolumn{2}{c|}{} & user $1$ \\
            \cline{2-14}
            & \multicolumn{2}{c|}{\cellcolor{gray!50}} & 
            \multicolumn{2}{c|}{} & 
            \multicolumn{2}{c|}{} & 
            \multicolumn{2}{c|}{\cellcolor{gray!50}} & \multicolumn{2}{c|}{\cellcolor{gray!50}} & \multicolumn{2}{c|}{} & user $2$ \\
            \cline{2-14}
            & \multicolumn{2}{c|}{} & 
            \multicolumn{2}{c|}{\cellcolor{gray!50}} & 
            \multicolumn{2}{c|}{} & 
            \multicolumn{2}{c|}{\cellcolor{gray!50}} & \multicolumn{2}{c|}{} & \multicolumn{2}{c|}{\cellcolor{gray!50}} & user $3$ \\
            \cline{2-14}
            & \multicolumn{2}{c|}{} & 
            \multicolumn{2}{c|}{} & 
            \multicolumn{2}{c|}{\cellcolor{gray!50}} & 
            \multicolumn{2}{c|}{} & \multicolumn{2}{c|}{\cellcolor{gray!50}} & \multicolumn{2}{c|}{\cellcolor{gray!50}} & user $4$ \\
            \hline
            \multicolumn{14}{c}{}\\[-0.7em]
        \end{tabular}  \\
        \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
            \cline{2-13}
            \multicolumn{1}{c|}{} & \multicolumn{3}{c|}{\tiny$\;\quad W_{123}(j) \,\quad$} & \multicolumn{3}{|c}{\tiny$\;\quad W_{124}(j) \,\quad$} & \multicolumn{3}{|c}{\tiny$\;\quad W_{134}(j) \,\quad$} & \multicolumn{3}{|c|}{\tiny$\;\quad W_{234}(j) \,\quad$} \\
            \hline
            \multirow{4}{*}{\rotatebox[origin=c]{90}{\small $j=3$}} & \multicolumn{3}{c|}{\cellcolor{gray!50}} & 
            \multicolumn{3}{c|}{\cellcolor{gray!50}} & 
            \multicolumn{3}{c|}{\cellcolor{gray!50}} & 
            \multicolumn{3}{c|}{} & user $1$ \\
            \cline{2-14}
            & \multicolumn{3}{c|}{\cellcolor{gray!50}} & 
            \multicolumn{3}{c|}{\cellcolor{gray!50}} & 
            \multicolumn{3}{c|}{} & 
            \multicolumn{3}{c|}{\cellcolor{gray!50}} & user $2$ \\
            \cline{2-14}
            & \multicolumn{3}{c|}{\cellcolor{gray!50}} & 
            \multicolumn{3}{c|}{} & 
            \multicolumn{3}{c|}{\cellcolor{gray!50}} & 
            \multicolumn{3}{c|}{\cellcolor{gray!50}} & user $3$ \\
            \cline{2-14}
            & \multicolumn{3}{c|}{} & 
            \multicolumn{3}{c|}{\cellcolor{gray!50}} & 
            \multicolumn{3}{c|}{\cellcolor{gray!50}} & 
            \multicolumn{3}{c|}{\cellcolor{gray!50}} & user $4$ \\
            \hline
        \end{tabular}
    \end{tabular}%
    }
    \caption{Cache placement visualization for Example~\ref{exmp:placement}.}
    \label{fig:cache pool}
\end{figure}

==> Uneven Cache Placement - ISIT _extend/SimResults.tex <==
\label{sec:simulation}
We use numerical simulations to evaluate the performance of the proposed location-dependent scheme. For simulations, we consider a $5m \times 5m$ square room where the transmitter is located in the middle of the room at a height of $3m$. The transmitter power is $30\mathrm{dB}$, the room area is split into $S=121$ states, and the users are uniformly distributed over the states. We compare the delivery time of the proposed scheme with unicasting and the baseline scheme of~\cite{tolli2017multi}. These delivery times are denoted by $T_m$, $T_u$ and $T_x$, respectively. For the scheme of~\cite{tolli2017multi}, $m(j) = \frac{M}{S}$ for every state $j \in \CS$, and the multicast rate for a user set $\CU$ is limited by $\min_{i \in \CU}r(s_i)$.

%For better comparison, we also consider the baseline caching scheme in~\cite{tolli2017multi}, for which $m(j) = \frac{M}{S}$ for every $j \in \CS$, and the delivery time $T_x$ for a user set $\CU$ is limited by $\min_{i \in \CU}r(s_i)$. 

%To evaluate the proposed method, we have carried out MATLAB simulations to compare the multicasting approach with the traditional unicasting method. We consider a $5 \times 5$ [$m^2$] square room where the transmitter is placed in the middle of the room on the ceiling (height is $3$ meters). The transmitter power is set to be $30$dB and the room is divided into $11 \times 11$ location matrix i.e., $S= 121$ (see figure~\ref{fig:system-model}). At each time slot, users are positioned in random locations using a uniform PDF.

In Figure~\ref{fig:timegain_Kx}, we have compared the proposed location-dependent scheme with unicast transmission, for different values of the user count parameter $K$. Clearly, the new scheme not only reduces the delivery time, but also makes it (almost) independent of $K$. This independence is justified by Theorem~\ref{theorem:proposed transmission time}, which states that for integer $\hat{t}$, $T_m$ is proportional to $\frac{K}{\hat{t}+1}$. However, as $\hat{t}=\min_{u_i\in\CK} t_i$ and $t_i = K m(s_i)$, as $K$ becomes larger, the value of $T_m$ approaches a constant value.

%Fig.~\ref{fig:time_K} shows the transmission time for the two methods mentioned earlier for different user numbers ($K$). As illustrated, the proposed method keeps the transmission time almost constant for different numbers of users ($K$). Note that for an integer $t_s$, the total transmission time for the proposed method is expressed as $\frac{K}{t_c + 1} C$~\eqref{eq:proposed transmission time}, where $t_c = \min\limits_{u_j \in \CK}t_j$, and $t_j = Km_j$. Therefore, for large $K$, the proposed method's total transmission time converges to $\lim T_m = \frac{1}{\zeta} C$, where $\zeta$ is some constant. As depicted in Fig.~\ref{fig:time_K}, the proposed method's transmission time stays within a constant amount for general values of $t_i$ and $K$. 

%Fig.~\ref{fig:timegain_K} shows the relative ratio $\frac{T_u}{T_m}$, where $T_u$ and $T_m$ denote the total transmission time of the \textit{unicasting} and \textit{multicasting} methods, respectively. Considering ~\eqref{eq:tm/tu}, simulation results agree with the analytical expression for integer $t_i$.

In Figure~\ref{fig:time_Mxs121}, the same comparison is done for different values of the cache size parameter $M$. It can be seen that the relative transmission gain $\frac{T_u}{T_m}$ increases almost linearly when $M > 0.4$. This is because for $M < 0.4$, there exists at least one state $j\in\CS$ for which $t(j) < 1$, and hence, the efficiency of the proposed scheme is reduced as multicasting is not possible when some users are located in such states. On the other hand, it can be seen that the proposed scheme performs worse than the baseline scheme of~\cite{tolli2017multi} when $M$ is small.
%since the proposed scheme highly depends on the users' local caching gains, for small $M$, it performs worse than the baseline scheme of~\cite{tolli2017multi}. 
This is because our proposed scheme sacrifices the global caching gain for a higher local caching gain. While this may not seem appealing, it results in more resilient performance if the ratio between the best and worst channel conditions is large. This is investigated in Figure~\ref{fig:timegain_Mx441}, where we have repeated the simulations for a larger room area of $10m \times 10m$, split into $S=441$ states. Clearly, in this case, the proposed location-dependent scheme outperforms the baseline scheme of~\cite{tolli2017multi} with a good margin, confirming its resilience to the existence of ill-conditioned states. 
%which in turn provides more resilient performance for worst case scenarios as illustrated in Fig.~\ref{fig:timegain_Mx441}. 

%In Fig.~\ref{fig:timegain_Mx441}, We consider a larger room $10 \times 10 [m^2]$ to investigate more harsh conditions. As depicted, when there exist some $j \in \CS$ such that $r(j)$ is very low, uniform cache allocation of original CC scheme should be highly avoided. When users are located in ill-conditioned states, the transmission rate is highly reduced, limiting the CC performance. Such scenarios are well handled in the proposed scheme through memory allocation in~\eqref{cache-allocation}. As a result, local cache gain is more effective than the global caching gain in bottle-neck scenarios.



%Fig.~\ref{fig:time_M} shows the transmission time for the two methods mentioned earlier for different cache sizes ($M$). As illustrated, the proposed outperforms the traditional \textit{unicasting} scheme. Note that for $M < 40$, there exist some $s \in \mathcal{S}$ where $t_s < 1$. In such scenarios, the proposed method has a less effective gain as some contents are not cached by any user. Thus, these contents must be delivered using \textit{unicasting} scheme (the multicasting opportunity is not available). Finally, Fig.~\ref{fig:timegain_M} compares the relative ratio $\frac{T_u}{T_m}$ for different user cache size ($M$). 

%\begin{figure}
%    \centering 
%    \includegraphics[width=1\columnwidth,keepaspectratio]{Figs/time_Kg.eps}
%    \caption{Total transmission time for multicasting ($T_m$) and unicasting ($T_u$) for different number of users $K$.}
%\label{fig:time_K}
%\end{figure}

%\begin{figure}
%    \centering 
%    \includegraphics[width=1\columnwidth,keepaspectratio]{Figs/timegain_Kg.eps}
%    \caption{Average relative gain ($\frac{T_u}{T_m}$) for different number of users $K$.}
%\label{fig:timegain_K}
%\end{figure}

%\begin{figure}
%    \centering 
%    \includegraphics[width=1\columnwidth,keepaspectratio]{Figs/time_Mg.eps}
%    \caption{Total transmission time for multicasting ($T_m$) and unicasting ($T_u$) for different users' cache size ($M$).}
%\label{fig:time_M}
%\end{figure}

%\begin{figure}
%    \centering 
%    \includegraphics[width=1\columnwidth,keepaspectratio]{Figs/timegain_Mg.eps}
%    \caption{Average relative gain ($\frac{T_u}{T_m}$) for different users' cache size ($M$).}
%\label{fig:timegain_M}
%\end{figure}

%\begin{figure}
%    \centering 
%    \includegraphics[width=1\columnwidth,keepaspectratio]{Figs/time_Kx.eps}
%    \caption{Average delivery time for different number of users $K$, where $M = \frac{3}{4}S$.}
%\label{fig:timegain_Kx}
%\end{figure}

%\begin{figure}
%    \centering 
%    \includegraphics[width=1\columnwidth,keepaspectratio]{Figs/timegain_mx_g.eps}
%    \caption{Average relative gain $\{\frac{T_u}{T_m}, \frac{T_u}{T_x}\}$ for different users' cache size ($M$), where $K = 10$ and $S = 121$.}
%\label{fig:time_Mxs121}
%\end{figure}

%\begin{figure}
%    \centering 
%    \includegraphics[width=1\columnwidth,keepaspectratio]{Figs/timegain_mx_g_S441.eps}
%    \caption{Average relative gain $\{\frac{T_u}{T_m}, \frac{T_u}{T_x}\}$ for different users' cache size ($M$), where $K = 10$ and $S = 441$.}
%\label{fig:timegain_Mx441}
%\end{figure}


==> Uneven Cache Placement - ISIT _extend/SysModel.tex <==
We envision a bounded environment (game hall, operating theatre, etc.) in which a single-antenna server serves $K$ single-antenna users through wireless communication links. The set of users is denoted by $\CK = \{ 1, ..., K \}$. The users are equipped with finite-size cache memories and are free to move throughout the environment. At each time slot, every user requests data from the server based on the application needs and its location. The requested data content can be divided into static and dynamic parts where the former can be proactively stored in the user cache memories. This paper focuses on the wireless delivery of the static location-dependent content partially aided by in-device cache memories.\footnote{We assume that a portion of the achievable data rate available at each user is dedicated to deliver the dynamic content without cache assistance.} A real-world application of this communication setup is a wireless immersive digital experience environment where the requested data is needed for reconstructing the location-dependent 3D field-of-view (FoV) at each user. The goal is to design a cache-aided communication scheme that minimizes the maximum required delivery time to transmit all the requested data to the served users. In other words, the aim is to provide a uniform QoE, irrespective of the users' location.

Intuitively, a larger share of the total cache memory should be reserved for storing data needed in locations where the communication quality is poor. We split the environment into $S$ regions, such that all points in a given region have almost the same distance from the server (i.e., can be served approximately with the same data rate). In the following, we refer to these regions as states and denote the set of states as $\CS$. A graphical example of an application environment with its states is provided in Figure~\ref{fig:system-model}. The file required for reconstructing the FoV of state $j \in \CS$ is denoted by $W(j)$. We assume for every region $j\in\CS$, the size of $W(j)$ is $F$ bits, and every user is equipped with a cache memory of size $MF$ bits. For the sake of simplicity, we consider a normalized data unit and drop $F$ in subsequent notations. Moreover, we consider the delivery procedure in a specific time slot and ignore the time index (the same procedure is repeated every time slot).

We assume a wideband communication scheme, where the total bandwidth is divided into several small frequency bins. %Assuming large enough bandwidth, the number of contained fading variations will be enough to apply the law of large numbers. 
For simplicity, we assume that the attainable expected rate at a particular location roughly depends on the transmitted power and the distance between the location and the server. Thus, the expected data rate attained in state $j\in \CS$ is expressed as
%\begin{equation} \label{eq: state-rate}
    $\bar{r}(j) = \log(1+\frac{P d^{-n}(j)}{N_0})$,
%\end{equation}
where $P$ is the transmission power, $N_0$ is the additive white Gaussian noise power, $n$ is the path-loss component, and $d(j)$ is the maximum distance from the server to all the points in state $j$.\footnote{
We need an estimation of the achievable rate at different states to perform the location-dependent cache placement. However, during the delivery phase, the communication can be performed with real achievable rates calculated using the available channel state information (CSI). In this paper, for notational and analysis simplicity, we have assumed the proposed rate estimation in the placement phase, based on the simple path loss model and line of sight (LOS) communications, is also valid throughout the delivery phase. Relaxing this assumption is left for the extended version of the paper.
%In the line-of-sight (LOS) scenario, since the server knows the path-loss exponent and the worst-case distance related to a state, it deduces the state's rate for data transmission. For non-line-of-sight (NLoS), to encounter any randomness due to large- and small-scale fading components, a training phase is required. In the training phase, the server calculates the least achievable rate for each state based on the received signal strength (RSS). The user's excessive achievable rate can be reserved for transmission of the dynamic data part.
} Thus, the expected data rate over all the frequency bins is approximated as $\hat{r}(j) \sim B\bar{r}(j)$, where $B$ is the communication bandwidth. For ease of exposition, we consider normalized data rate, i.e., $r(j) = \frac{\hat{r}(j)}{F}$, throughout this paper.
%where $d_i$ is the user-server distance of user $i \in \CK$, $n$ is the path-loss component, and $G$ is a $\mathbb{CN}(0,1)$ random variable.

%For the sake of simplicity, we consider the delivery procedure in a specific time instant and ignore the time index (the same procedure is repeated for all the time instants). The requested data may be delivered through unicasting in a TDMA fashion or multicasting to multiple users in a single transmission. 

\begin{figure}
    \centering 
    \includegraphics[width=0.8\columnwidth,keepaspectratio]{Figs/system_model2.pdf}
    \caption{An application environment with $K=3$ users, split into $S=8$ states. $r(j)$ is the state-specific achievable rate and $r(3) > r(2) > r(7)$. $X_{123}$ is the multicast message, and $Y_i$ represents the data part intended for user $i$. The black bar below each user indicates how much of the requested data is cached, and $*$ denotes the variable-rate NCM operation.}
    \label{fig:system-model}
\end{figure}


==> Uneven Cache Placement - ISIT _extend/abbrev.tex <==
%!TeX root = d2d-cc.tex

% Declaration of the abbreviations
\DeclareAcronym{ADMM}{
    short = ADMM,
    long = alternating direction method of multipliers,
    list = Alternating Direction Method of Multipliers,
    class = abbrev
}

\DeclareAcronym{MGMC}{
    short = MGMC,
    long = multi-group multi-casting,
    list = multi-group multi-casting,
    class = abbrev
}

\DeclareAcronym{SGMC}{
    short = SGMC,
    long = single-group multi-casting,
    list = single-group multi-casting,
    class = abbrev
}
\DeclareAcronym{AoA}{
    short = AoA,
    long = angle-of-arrival,
    list = Angle-of-Arrival,
    class = abbrev
}

\DeclareAcronym{AoD}{
    short = AoD,
    long = angle-of-departure,
    list = Angle-of-Departure,
    class = abbrev
}

\DeclareAcronym{KKT}{
    short = KKT,
    long = Karush-Kuhn-Tucker,
    list = Karush-Kuhn-Tucker,
    class = abbrev
}

\DeclareAcronym{MMF}{
    short = MMF,
    long = max-min-fairness,
    list = max-min-fairness,
    class = abbrev
}

\DeclareAcronym{BB}{
    short = BB,
    long = base band,
    list = Base Band,
    class = abbrev
}

\DeclareAcronym{BC}{
    short = BC,
    long = broadcast channel,
    list = Broadcast Channel,
    class = abbrev
}

\DeclareAcronym{BS}{
    short = BS,
    long = base station,
    list = Base Station,
    class = abbrev
}

\DeclareAcronym{BR}{
    short = BR,
    long = best response,
    list = Best Response, 
    class = abbrev
}

\DeclareAcronym{CB}{
    short = CB,
    long = coordinated beamforming,
    list = Coordinated Beamforming,
    class = abbrev
}

\DeclareAcronym{CC}{
    short = CC,
    long = coded caching,
    list = Coded Caching,
    class = abbrev
}

\DeclareAcronym{CE}{
    short = CE,
    long = channel estimation,
    list = Channel Estimation,
    class = abbrev
}

\DeclareAcronym{CoMP}{
    short = CoMP,
    long = coordinated multi-point transmission,
    list = Coordinated Multi-Point Transmission,
    class = abbrev
}

\DeclareAcronym{CRAN}{
    short = C-RAN,
    long = cloud radio access network,
    list = Cloud Radio Access Network,
    class = abbrev
}

\DeclareAcronym{CSE}{
    short = CSE,
    long = channel specific estimation,
    list = Channel Specific Estimation,
    class = abbrev
}

\DeclareAcronym{CSI}{
    short = CSI,
    long = channel state information,
    list = Channel State Information,
    class = abbrev
}

\DeclareAcronym{CSIT}{
    short = CSIT,
    long = channel state information at the transmitter,
    list = Channel State Information at the Transmitter,
    class = abbrev
}

\DeclareAcronym{CU}{
    short = CU,
    long = central unit,
    list = Central Unit,
    class = abbrev
}

\DeclareAcronym{D2D}{
    short = D2D,
    long = device-to-device,
    list = Device-to-Device,
    class = abbrev
}

\DeclareAcronym{DE-ADMM}{
    short = DE-ADMM,
    long = direct estimation with alternating direction method of multipliers,
    list = Direct Estimation with Alternating Direction Method of Multipliers,
    class = abbrev
}

\DeclareAcronym{DE-BR}{
    short = DE-BR,
    long = direct estimation with best response,
    list = Direct Estimation with Best Response,
    class = abbrev
}

\DeclareAcronym{DE-SG}{
    short = DE-SG,
    long = direct estimation with stochastic gradient,
    list = Direct Estimation with Stochastic Gradient,
    class = abbrev
}

\DeclareAcronym{DFT}{
	short = DFT,
	long = discrete fourier transform,
	list = Discrete Fourier Transform,
	class = abbrev
}

\DeclareAcronym{DoF}{
    short = DoF,
    long = degrees of freedom,
    list = Degrees of Freedom,
    class = abbrev
}

\DeclareAcronym{DL}{
    short = DL,
    long = downlink,
    list = Downlink,
    class = abbrev
}

\DeclareAcronym{GD}{
	short = GD, 
	long = gradient descent,
	list = Gradeitn Descent,
	class = abbrev
}

\DeclareAcronym{IBC}{
    short = IBC,
    long = interfering broadcast channel,
    list = Interfering Broadcast Channel,
    class = abbrev
}

\DeclareAcronym{i.i.d.}{
    short = i.i.d.,
    long = independent and identically distributed,
    list = Independent and Identically Distributed,
    class = abbrev
}

\DeclareAcronym{JP}{
    short = JP,
    long = joint processing,
    list = Joint Processing,
    class = abbrev
}


\DeclareAcronym{LOS}{
	short = LOS,
	long = line-of-sight,
	list = Line-of-Sight,
	class = abbrev
}

\DeclareAcronym{LS}{
    short = LS,
    long = least squares,
    list = Least Squares,
    class = abbrev
}

\DeclareAcronym{LTE}{
    short = LTE,
    long = Long Term Evolution,
    class = abbrev
}

\DeclareAcronym{LTE-A}{
    short = LTE-A,
    long = Long Term Evolution Advanced,
    class = abbrev
}

\DeclareAcronym{MIMO}{
    short = MIMO,
    long = multiple-input multiple-output,
    list = Multiple-Input Multiple-Output,
    class = abbrev
}

\DeclareAcronym{MISO}{
    short = MISO,
    long = multiple-input single-output,
    list = Multiple-Input Single-Output,
    class = abbrev
}

\DeclareAcronym{MSE}{
    short = MSE,
    long = mean-squared error,
    list = Mean-Squared Error,
    class = abbrev
}

\DeclareAcronym{MMSE}{
    short = MMSE,
    long = minimum mean-squared error,
    list = Minimum Mean-Squared Error,
    class = abbrev
}

\DeclareAcronym{mmWave}{
	short = mmWave,
	long = millimeter wave,
	list = Millimeter Wave,
	class = abbrev
}

\DeclareAcronym{MU-MIMO}{
    short = MU-MIMO,
    long = multi-user \ac{MIMO},
    list = Multi-User \ac{MIMO},
    class = abbrev
}

\DeclareAcronym{OTA}{
    short = OTA,
    long = over-the-air,
    list = Over-the-Air,
    class = abbrev
}

\DeclareAcronym{PSD}{
    short = PSD,
    long = positive semidefinite,
    list = Positive Semidefinite,
    class = abbrev
}

\DeclareAcronym{QoS}{
	short = QoS,
	long = quality of service,
	list = Quality of Service,
	class = abbrev
}

\DeclareAcronym{RCP}{
	short = RCP,
	long = remote central processor,
	list = Remote Central Processor,
	class = abbrev
}

\DeclareAcronym{RRH}{
    short = RRH,
    long = remote radio head,
    list = Remote Radio Head,
    class = abbrev
}

\DeclareAcronym{RSSI}{
    short = RSSI,
    long = received signal strength indicator,
    list = Received Signal Strength Indicator,
    class = abbrev
}

\DeclareAcronym{RX}{
	short = RX,
	long = receiver,
	list = Receiver,
	class = abbrev
}

\DeclareAcronym{SCA}{
    short = SCA,
    long = successive-convex-approximation,
    list = Successive-Convex-Approximation,
    class = abbrev
}

\DeclareAcronym{SG}{
    short = SG,
    long = stochastic gradient,
    list = Stochastic Gradient,
    class = abbrev
}

\DeclareAcronym{SNR}{
    short = SNR,
    long = signal-to-noise-ratio,
    list = Signal-to-Noise Ratio,
    class = abbrev
}

\DeclareAcronym{SDR}{
    short = SDR,
    long = semi-definite-relaxation,
    list = semi-definite-relaxation,
    class = abbrev
}

\DeclareAcronym{SINR}{
    short = SINR,
    long = signal-to-interference-plus-noise ratio,
    list = Signal-to-Interference-plus-Noise Ratio,
    class = abbrev
}

\DeclareAcronym{SOCP}{
	short = SOCP, 
	long = second order cone program,
	list = Second Order Cone Program,
	class = abbrev
}

\DeclareAcronym{SSE}{
    short = SSE,
    long = stream specific estimation,
    list = Stream Specific Estimation,
    class = abbrev
}

\DeclareAcronym{SVD}{
	short = SVD,
	long = singular value decomposition,
	list = Singular Value Decomposition,
	class = abbrev
}

\DeclareAcronym{TDD}{
	short = TDD,
	long = time division duplex,
	list = Time Division Duplex,
	class = abbrev
}

\DeclareAcronym{TX}{
	short = TX,
	long = transmitter,
	list = Transmitter,
	class = abbrev
}

\DeclareAcronym{UE}{
    short = UE,
    long = user equipment,
    list = User Equipment,
    class = abbrev
}

\DeclareAcronym{UL}{
    short = UL,
    long = uplink,
    list = Uplink,
    class = abbrev
}

\DeclareAcronym{ULA}{
	short = ULA,
	long = uniform linear array,
	list = Uniform Linear Array,
	class = abbrev
}

\DeclareAcronym{NCM}{
	short = NCM,
	long = nested code modulation,
	list = nested code modulation,
	class = abbrev
}

\DeclareAcronym{UPA}{
    short = UPA,
    long = uniform planar array,
    list = Uniform Planar Array,
    class = abbrev
}

\DeclareAcronym{WMMSE}{
    short = WMMSE,
    long = weighted minimum mean-squared error,
    list = Weighted Minimum Mean-Squared Error,
    class = abbrev
}

\DeclareAcronym{WMSEMin}{
    short = WMSEMin,
    long = weighted sum \ac{MSE} minimization,
    list = Weighted sum \ac{MSE} Minimization,
    class = abbrev
}

\DeclareAcronym{WBAN}{
	short = WBAN,
	long = wireless body area network,
	list = Wireless Body Area Network,
	class = abbrev
}

\DeclareAcronym{WSRMax}{
    short = WSRMax,
    long = weighted sum rate maximization,
    list = Weighted Sum Rate Maximization,
    class = abbrev
}

==> abbrev.tex <==
%!TeX root = d2d-cc.tex

% Declaration of the abbreviations
\DeclareAcronym{ADMM}{
    short = ADMM,
    long = alternating direction method of multipliers,
    list = Alternating Direction Method of Multipliers,
    class = abbrev
}

\DeclareAcronym{MGMC}{
    short = MGMC,
    long = multi-group multi-casting,
    list = multi-group multi-casting,
    class = abbrev
}

\DeclareAcronym{SGMC}{
    short = SGMC,
    long = single-group multi-casting,
    list = single-group multi-casting,
    class = abbrev
}
\DeclareAcronym{AoA}{
    short = AoA,
    long = angle-of-arrival,
    list = Angle-of-Arrival,
    class = abbrev
}

\DeclareAcronym{AoD}{
    short = AoD,
    long = angle-of-departure,
    list = Angle-of-Departure,
    class = abbrev
}

\DeclareAcronym{KKT}{
    short = KKT,
    long = Karush-Kuhn-Tucker,
    list = Karush-Kuhn-Tucker,
    class = abbrev
}

\DeclareAcronym{MMF}{
    short = MMF,
    long = max-min-fairness,
    list = max-min-fairness,
    class = abbrev
}

\DeclareAcronym{BB}{
    short = BB,
    long = base band,
    list = Base Band,
    class = abbrev
}

\DeclareAcronym{BC}{
    short = BC,
    long = broadcast channel,
    list = Broadcast Channel,
    class = abbrev
}

\DeclareAcronym{BS}{
    short = BS,
    long = base station,
    list = Base Station,
    class = abbrev
}

\DeclareAcronym{BR}{
    short = BR,
    long = best response,
    list = Best Response, 
    class = abbrev
}

\DeclareAcronym{CB}{
    short = CB,
    long = coordinated beamforming,
    list = Coordinated Beamforming,
    class = abbrev
}

\DeclareAcronym{CC}{
    short = CC,
    long = coded caching,
    list = Coded Caching,
    class = abbrev
}

\DeclareAcronym{CE}{
    short = CE,
    long = channel estimation,
    list = Channel Estimation,
    class = abbrev
}

\DeclareAcronym{CoMP}{
    short = CoMP,
    long = coordinated multi-point transmission,
    list = Coordinated Multi-Point Transmission,
    class = abbrev
}

\DeclareAcronym{CRAN}{
    short = C-RAN,
    long = cloud radio access network,
    list = Cloud Radio Access Network,
    class = abbrev
}

\DeclareAcronym{CSE}{
    short = CSE,
    long = channel specific estimation,
    list = Channel Specific Estimation,
    class = abbrev
}

\DeclareAcronym{CSI}{
    short = CSI,
    long = channel state information,
    list = Channel State Information,
    class = abbrev
}

\DeclareAcronym{CSIT}{
    short = CSIT,
    long = channel state information at the transmitter,
    list = Channel State Information at the Transmitter,
    class = abbrev
}

\DeclareAcronym{CU}{
    short = CU,
    long = central unit,
    list = Central Unit,
    class = abbrev
}

\DeclareAcronym{D2D}{
    short = D2D,
    long = device-to-device,
    list = Device-to-Device,
    class = abbrev
}

\DeclareAcronym{DE-ADMM}{
    short = DE-ADMM,
    long = direct estimation with alternating direction method of multipliers,
    list = Direct Estimation with Alternating Direction Method of Multipliers,
    class = abbrev
}

\DeclareAcronym{DE-BR}{
    short = DE-BR,
    long = direct estimation with best response,
    list = Direct Estimation with Best Response,
    class = abbrev
}

\DeclareAcronym{DE-SG}{
    short = DE-SG,
    long = direct estimation with stochastic gradient,
    list = Direct Estimation with Stochastic Gradient,
    class = abbrev
}

\DeclareAcronym{DFT}{
	short = DFT,
	long = discrete fourier transform,
	list = Discrete Fourier Transform,
	class = abbrev
}

\DeclareAcronym{DoF}{
    short = DoF,
    long = degrees of freedom,
    list = Degrees of Freedom,
    class = abbrev
}

\DeclareAcronym{DL}{
    short = DL,
    long = downlink,
    list = Downlink,
    class = abbrev
}

\DeclareAcronym{GD}{
	short = GD, 
	long = gradient descent,
	list = Gradeitn Descent,
	class = abbrev
}

\DeclareAcronym{IBC}{
    short = IBC,
    long = interfering broadcast channel,
    list = Interfering Broadcast Channel,
    class = abbrev
}

\DeclareAcronym{i.i.d.}{
    short = i.i.d.,
    long = independent and identically distributed,
    list = Independent and Identically Distributed,
    class = abbrev
}

\DeclareAcronym{JP}{
    short = JP,
    long = joint processing,
    list = Joint Processing,
    class = abbrev
}


\DeclareAcronym{LOS}{
	short = LOS,
	long = line-of-sight,
	list = Line-of-Sight,
	class = abbrev
}

\DeclareAcronym{LS}{
    short = LS,
    long = least squares,
    list = Least Squares,
    class = abbrev
}

\DeclareAcronym{LTE}{
    short = LTE,
    long = Long Term Evolution,
    class = abbrev
}

\DeclareAcronym{LTE-A}{
    short = LTE-A,
    long = Long Term Evolution Advanced,
    class = abbrev
}

\DeclareAcronym{MIMO}{
    short = MIMO,
    long = multiple-input multiple-output,
    list = Multiple-Input Multiple-Output,
    class = abbrev
}

\DeclareAcronym{MISO}{
    short = MISO,
    long = multiple-input single-output,
    list = Multiple-Input Single-Output,
    class = abbrev
}

\DeclareAcronym{MSE}{
    short = MSE,
    long = mean-squared error,
    list = Mean-Squared Error,
    class = abbrev
}

\DeclareAcronym{MMSE}{
    short = MMSE,
    long = minimum mean-squared error,
    list = Minimum Mean-Squared Error,
    class = abbrev
}

\DeclareAcronym{mmWave}{
	short = mmWave,
	long = millimeter wave,
	list = Millimeter Wave,
	class = abbrev
}

\DeclareAcronym{MU-MIMO}{
    short = MU-MIMO,
    long = multi-user \ac{MIMO},
    list = Multi-User \ac{MIMO},
    class = abbrev
}

\DeclareAcronym{OTA}{
    short = OTA,
    long = over-the-air,
    list = Over-the-Air,
    class = abbrev
}

\DeclareAcronym{PSD}{
    short = PSD,
    long = positive semidefinite,
    list = Positive Semidefinite,
    class = abbrev
}

\DeclareAcronym{QoS}{
	short = QoS,
	long = quality of service,
	list = Quality of Service,
	class = abbrev
}

\DeclareAcronym{RCP}{
	short = RCP,
	long = remote central processor,
	list = Remote Central Processor,
	class = abbrev
}

\DeclareAcronym{RRH}{
    short = RRH,
    long = remote radio head,
    list = Remote Radio Head,
    class = abbrev
}

\DeclareAcronym{RSSI}{
    short = RSSI,
    long = received signal strength indicator,
    list = Received Signal Strength Indicator,
    class = abbrev
}

\DeclareAcronym{RX}{
	short = RX,
	long = receiver,
	list = Receiver,
	class = abbrev
}

\DeclareAcronym{SCA}{
    short = SCA,
    long = successive-convex-approximation,
    list = Successive-Convex-Approximation,
    class = abbrev
}

\DeclareAcronym{SG}{
    short = SG,
    long = stochastic gradient,
    list = Stochastic Gradient,
    class = abbrev
}

\DeclareAcronym{SNR}{
    short = SNR,
    long = signal-to-noise-ratio,
    list = Signal-to-Noise Ratio,
    class = abbrev
}

\DeclareAcronym{SDR}{
    short = SDR,
    long = semi-definite-relaxation,
    list = semi-definite-relaxation,
    class = abbrev
}

\DeclareAcronym{SINR}{
    short = SINR,
    long = signal-to-interference-plus-noise ratio,
    list = Signal-to-Interference-plus-Noise Ratio,
    class = abbrev
}

\DeclareAcronym{SOCP}{
	short = SOCP, 
	long = second order cone program,
	list = Second Order Cone Program,
	class = abbrev
}

\DeclareAcronym{SSE}{
    short = SSE,
    long = stream specific estimation,
    list = Stream Specific Estimation,
    class = abbrev
}

\DeclareAcronym{SVD}{
	short = SVD,
	long = singular value decomposition,
	list = Singular Value Decomposition,
	class = abbrev
}

\DeclareAcronym{TDD}{
	short = TDD,
	long = time division duplex,
	list = Time Division Duplex,
	class = abbrev
}

\DeclareAcronym{TX}{
	short = TX,
	long = transmitter,
	list = Transmitter,
	class = abbrev
}

\DeclareAcronym{UE}{
    short = UE,
    long = user equipment,
    list = User Equipment,
    class = abbrev
}

\DeclareAcronym{UL}{
    short = UL,
    long = uplink,
    list = Uplink,
    class = abbrev
}

\DeclareAcronym{ULA}{
	short = ULA,
	long = uniform linear array,
	list = Uniform Linear Array,
	class = abbrev
}

\DeclareAcronym{NCM}{
	short = NCM,
	long = nested code modulation,
	list = nested code modulation,
	class = abbrev
}

\DeclareAcronym{UPA}{
    short = UPA,
    long = uniform planar array,
    list = Uniform Planar Array,
    class = abbrev
}

\DeclareAcronym{WMMSE}{
    short = WMMSE,
    long = weighted minimum mean-squared error,
    list = Weighted Minimum Mean-Squared Error,
    class = abbrev
}

\DeclareAcronym{WMSEMin}{
    short = WMSEMin,
    long = weighted sum \ac{MSE} minimization,
    list = Weighted sum \ac{MSE} Minimization,
    class = abbrev
}

\DeclareAcronym{WBAN}{
	short = WBAN,
	long = wireless body area network,
	list = Wireless Body Area Network,
	class = abbrev
}

\DeclareAcronym{WSRMax}{
    short = WSRMax,
    long = weighted sum rate maximization,
    list = Weighted Sum Rate Maximization,
    class = abbrev
}
